An Optimization algorithm for nonsmooth nonconvex problems with upper-C^2 objective

An optimization algorithm for nonsmooth nonconvex constrained optimization problems with upper-C2 objective functions is proposed and analyzed. Upper-C2 is a weakly concave property that exists in difference of convex (DC) functions and arises naturally in many applications, particularly certain classes of solutions to parametric optimization problems [34, 4], e.g., recourse of stochastic programming [36] and projection into closed sets [34]. The algorithm can be viewed as a bundle method specialized for upper-C2 problems and is globally convergent with bounded algorithm parameters. Compared to conventional bundle methods, the proposed method is both simpler and computationally more efficient. The algorithm handles general smooth constraints similarly to sequential quadratic programming (SQP) methods and uses a line search to ensure progress. The potential inconsistencies from the linearization of the constraints are addressed through a penalty method. The capabilities of the algorithm are demonstrated by solving both simple upper-C2 problems and real-world optimal power flow problems used in current power grid industry practices.

==> Sections_journal/Algorithm.tex <==
\section{\normalsize Simplified bundle algorithm}\label{sec:alg}
Given the nonsmooth nonconvex objective $r$ in~\eqref{eqn:opt-ms-simp}, we consider the bundle methods which have 
proven to be one of the most successful methods in solving such 
problems~\cite{lemarechal2001}. 
The proposed algorithm simplifies the bundle while retain many of the algorithm's features.
Motivated by the discussion in Section~\ref{sec:prob}, we make the following assumption. 
\begin{assumption}\label{assp:upperC2}
	The Lipschitz continuous objective $r$ in~\eqref{eqn:opt-ms-simp} is upper-$C^2$. 
\end{assumption}
\noindent In particular, inequality~\eqref{eqn:uppc2-def} is satisfied.
We point out that~\cite{noll2009,dao2015} have explored bundle methods and to our knowledge were the first to prove convergence for upper-$C^1$
objective and constraints. However, in their case the parameters of the approximation model are not guaranteed to be finite, in addition to the aforementioned challenges in applying bundle method to constrained optimization.
We assume uniform boundedness on the Hessian of the smooth constraints, a common assumption in literature~\cite{curtis2012}.
\begin{assumption}\label{assp:boundedHc}
	The constraints $c$ are twice differentiable. There exists a constant $H_u^c$ such that the Hessian of constraints $c$ satisfy $\frac{1}{2}x^T \nabla^2c_j(x) x \leq H_u^c\norm{x}^2$ for all feasible $x$ and $1\leq j\leq m$. 
\end{assumption}
Assumption~\ref{assp:boundedHc} can be relaxed to $c$ being strictly continuously differentiable.
\subsection{Algorithm description}\label{sec:alg-1}
The simplified bundle algorithm is an iterative method with locally approximated objective at each iteration. 
It bears similarity to SQP in the treatment of constraints and can be viewed as its extension.
Compared to conventional bundle methods, the local convex quadratic approximation $\phi_k(\cdot)$ to $r$  
is dependent only on the current serious point instead of a bundle of points. 
More specifically, at iteration $k$ and its serious step $x_k$, $\phi_k(\cdot)$ is
\begin{equation} \label{eqn:opt-rc-appx-x}
 \centering
  \begin{aligned}
	  \phi_k(x) = r(x_k) + g_k^T(x-x_k) + \frac{1}{2}\alpha_k \norm{x-x_k}^2,
  \end{aligned}
\end{equation}
where $g_k\in\bar{\partial} r(x_k)$, and $\alpha_k>0$ is the scalar quadratic coefficient.
Equivalently, denoting $d=x-x_k$, $\phi_k(x)$ can be reformulated as $\Phi_k(d)$ such that
\begin{equation} \label{eqn:opt-rc-appx}
 \centering
  \begin{aligned}
	  \Phi_k(d) &= r_k + g_k^T d +\frac{1}{2}\alpha_k\left\lVert d\right\rVert ^2,\\ 
  \end{aligned}
\end{equation}
where $r_k=r(x_k)$. The function 
value and subgradient at $x_k$ are exact, \textit{i.e.}, $\Phi_k(0)=r_k,\nabla\Phi_k(0)=g_k$.
%with  
%\begin{equation} \label{eqn:opt-rc-appx2}
% \centering
%  \begin{aligned}
%	  &\Phi_k(0) = r_k \textnormal{ and } \nabla \Phi_k (0) = g_k. 
%  \end{aligned}
%\end{equation}
Furthermore, the constraints in~\eqref{eqn:opt-ms-simp} are linearized. The subproblem to be solved 
at iteration $k$ is 
\begin{equation} \label{eqn:opt-ms-simp-bundle}
 \centering
  \begin{aligned}
   &\underset{\substack{d}}{\text{minimize}} 
	  & & \Phi_k(d)\\
   &\text{subject to}
	  & & c(x_k) + \nabla c(x_k)^T d= 0, \\
	  &&& d_l^k \leq d \leq d_u^k,
  \end{aligned}
\end{equation}
where $d_l^k=-x_k,d_u^k=x_u-x_k$.
As in SQP methods, it is possible that the linearized constraints 
cause problem~\eqref{eqn:opt-ms-simp-bundle} to be infeasible. 
One way to address this issue is presented in Section~\ref{sec:lincons}.
In this section, we operate under the assumption that~\eqref{eqn:opt-ms-simp-bundle} can be solved and 
its solution is denoted as $d_k$.
To measure progress in both the objective and constraints, 
the $l_1$ merit function is adopted:
\begin{equation} \label{eqn:opt-ms-simp-bundle-merit}
 \centering
  \begin{aligned}
	  \phi_{1\theta_k}(x) = r(x) + \theta_k \norm{c(x)}_1, \\
  \end{aligned}
\end{equation}
where $\norm{\cdot}_1$ is the 1-norm and $\theta_k>0$ is a penalty parameter. 
A line search step on the constraints is needed in order to ensure progress
in the merit function~\eqref{eqn:opt-ms-simp-bundle-merit}.
The predicted change on the objective is defined as 
\begin{equation} \label{def:pd}
 \centering
  \begin{aligned}
	  \delta_k =& \Phi_k(0) - \Phi_k(d_k) 
	   = -g_k^T d_k -\frac{1}{2}\alpha_k\norm{d_k}^2.
  \end{aligned}
\end{equation}
%The step $d_k$ is defined as $d_k=x_{k+1}-x_k$.
To measure whether the approximation model $\Phi_k(\cdot)$ of the objective formed at $x_k$ is still valid at the trial step $x_k+d_k$,
we define the ratio $\rho_k$ as
\begin{equation} \label{eqn:decrease-ratio-1}
 \centering
  \begin{aligned}
	  \rho_k = \begin{cases}
		  r(x_k)-r(x_k+d_k)-\eta_l^+ \delta_k, \ &\delta_k \geq 0,\\
		  r(x_k)-r(x_k+d_k)-\eta_l^- \delta_k, \  &\delta_k <0,
	  \end{cases}
  \end{aligned}
\end{equation}
where $0<\eta_l^+\leq1$ and $\eta_l^-\geq 1$ are two parameters of the algorithm. 
If $\rho_k>0$, the model is still valid and the algorithm proceeds to line search.
Otherwise, the trial step $x_k+d_k$ is 
rejected and the parameter $\alpha_k$ is updated to find a different trial step. This process 
draws inspiration from trust-region methods. 

The value of $\delta_k$ is not necessarily positive. Therefore, the 
corresponding threshold $\eta_l^+$ and $\eta_l^-$ differ based on the sign of $\delta_k$. 
In both cases, the actual change in the objective $r(x_k)-r(x_{k}+d_k)$ is allowed to
be slightly worse than the predicted one. 
This means that if $\delta_k\geq 0$, the actual decrease can be smaller than the predicted decrease $\delta_k$, 
though a fraction $\eta_l^+$ of  $\delta_k$ is required.
If $\delta_k<0$, 
the actual increase in objective value can be slightly larger than the predicted increase value $-\delta_k$, 
the degree to which is governed by $\eta_l^- \geq 1$.

%$\alpha_k$ while the decrease ratio for the merit function $\rho_{1k}$ is 
%\begin{equation} \label{eqn:decrease-ratio-merit}
% \centering
%  \begin{aligned}
%	  \rho_{1k} = \frac{\phi_{1k}(x_k,\theta_k)-\phi_{1k}(x_{k+1},\theta_k)  }{\Phi_k(x_k)+\theta_k \norm{c(x_k)}_1 - \Phi_k(x_{k+1})-\theta_k\norm{c(x_{k+1})}_1}.
%  \end{aligned}
%\end{equation}
Let the line search parameter be $\beta_k \in (0,1]$. Then, the serious step taken is given as 
$x_{k+1} = x_k + \beta_k d_k$.
Let $\delta_k^{\beta} = \Phi_k(0) - \Phi_k(\beta_k d_{k})$, we have  
\begin{equation} \label{def:pd2}
 \centering
  \begin{aligned}
	  \delta_k^{\beta} =& \Phi_k(0) - \Phi_k(\beta_k d_k)
	   = -\beta_k g_k^T d_k -\frac{1}{2}\beta_k^2 \alpha_k\norm{d_k}^2.
  \end{aligned}
\end{equation}
The predicted and actual change in objective at $x_{k+1}$ is measured by $\rho_k^{\beta}$ defined by
\begin{equation} \label{eqn:decrease-ratio-beta}
 \centering
  \begin{aligned}
	  \rho_k^{\beta} = \begin{cases}
		  r(x_k)-r(x_{k+1})-\eta_{\gamma}^+ \delta_k^{\beta}, \ & \delta_k^{\beta} \geq 0,\\
		  r(x_k)-r(x_{k+1})-\eta_{\gamma}^- \delta_k^{\beta} , \  & \delta_k^{\beta} <0.
	  \end{cases}
  \end{aligned}
\end{equation}
 The parameter $\eta_{\gamma}^{+}\in(0,1]$ and $\eta_{\gamma}^-\geq 1$ can have different values than $\eta_l^+$ and $\eta_l^-$ to increase  
 flexibility of the algorithm.
The first-order optimality conditions of subproblem~\eqref{eqn:opt-ms-simp-bundle} are
\begin{equation} \label{eqn:simp-bundle-KKT}
  \centering
   \begin{aligned}
	   g_k + \alpha_k d_k - \nabla c(x_k) \lambda^{k+1} -\zeta_l^{k+1}+\zeta_u^{k+1} =0,&\\
	   Z_u^{k+1}(d_k-d_u^k) = 0, Z_l^{k+1} (d_k-d_l^k) = 0,&\\
	   \lambda_j^{k+1}\left[c_j(x_k)+\nabla c_j(x_k)^T d_k\right] = 0,j=1,\dots,m,&\\
	   \zeta_u^{k+1},\zeta_l^{k+1},d_k -d_l^k,d_u^k-d_k\geq 0,&\\
	   c(x_k)+\nabla c(x_k)^Td_k= 0,&
   \end{aligned}
 \end{equation}
	where $\lambda^{k+1}\in \Rbb^m$ is the Lagrange multiplier for constraints $c$ and $\zeta_u^{k+1}$ and $\zeta_l^{k+1}\in \Rbb^n$ are the Lagrange multipliers for the bound constraints. 
	The matrices $Z_u^{k+1}$ and $Z_l^{k+1}$ are 
	diagonal matrices with values $\zeta_u^{k+1}$ and $\zeta_l^{k+1}$, respectively.
      An equivalent form of the complementarity conditions 
      of bound constraints based on $x_u$  is
\begin{equation} \label{eqn:simp-bundle-KKT-bound}
  \centering
   \begin{aligned}
	   Z_u^{k+1}(x_k+d_k-x_u) = 0, Z_l^{k+1} (x_k+d_k) &= 0,\\
	   \zeta_u^{k+1},\zeta_l^{k+1}, x_k+d_k ,x_u-x_k-d_k&\geq 0.\\
   \end{aligned}
 \end{equation}
\noindent The line search conditions are given as follows
\begin{equation} \label{eqn:line-search-cond}
 \centering
  \begin{aligned}
	  \theta_k \norm{c(x_k)}_1+\beta_k (\lambda^{k+1})^T c(x_k) &\geq \theta_k \norm{c(x_{k+1})}_1-\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2, \\
	  \theta_k \norm{c(x_k)}_1+\eta_{\gamma}^+ \beta_k (\lambda^{k+1})^T c(x_k) &\geq \theta_k \norm{c(x_{k+1})}_1-\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2, \\
	  \theta_k \norm{c(x_k)}_1+\eta_{\gamma}^- \beta_k (\lambda^{k+1})^T c(x_k) &\geq \theta_k \norm{c(x_{k+1})}_1-\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2. \\
  \end{aligned}
\end{equation}
The differences between the conditions are the parameters $\eta_{\gamma}^+$ and $\eta_{\gamma}^-$ in the second and third inequalities, which stem from the unknown sign of $\delta_k$ and $\delta_k^{\beta}$. 
For simplicity in implementation and analysis, we use the following alternative 
condition 
\begin{equation} \label{eqn:line-search-cond-alt}
 \centering
  \begin{aligned}
	  \theta_k \norm{c(x_k)}_1 - \eta_{\gamma}^-  \beta_k\left| (\lambda^{k+1})^T c(x_k)\right| &\geq \theta_k \norm{c(x_{k+1})}_1-\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2. \\
  \end{aligned}
\end{equation}
We will show that condition~\eqref{eqn:line-search-cond-alt} implies conditions in~\eqref{eqn:line-search-cond} in Lemma~\ref{lem:line-search-alt}.
%		  %
The simplified bundle method is presented in Algorithm~\ref{alg:simp-bundle}, where $\norm{\cdot}_{\infty}$ 
is the infinity norms. The terms for consistency restoration such as $\pi_{k-1}$ are explained in Section~\ref{sec:lincons}.
\begin{algorithm}
% \DontPrintSemicolon
% \SetAlgoNoLine 
   \caption{Simplified bundle method}\label{alg:simp-bundle}
	\begin{algorithmic}[1]
	    \STATE{Initialize $x_0$, $\alpha_0$, stopping error tolerance $\epsilon$, and $k=1$.
	Choose scalars $0<\eta_l^+\leq 1$, $0<\eta_{\beta}<\eta_{\gamma}^+\leq 1$, $\eta_l^-\geq 1$,$\eta_{\gamma}^-\geq 1$, $\eta_{\alpha}>1$ and $\gamma>0$. 
	    Evaluate the function value $r(x_0)$ and subgradient $g_0$.}
	\FOR{$k=0,1,2,...$}
	  \STATE{Form the quadratic function $\Phi_k$ in~\eqref{eqn:opt-rc-appx} and solve 
		subproblem~\eqref{eqn:opt-ms-simp-bundle} to obtain $d_{k}$ and Lagrange multiplier $\lambda^{k+1}$. (If constraints are inconsistent, enter consistency restoration Algorithm~\ref{alg:simp-bundle-const}. Then, go back to step 2 with $k=k+1$.)}
	  \IF{$\norm{d_k}\leq \epsilon$}
	    \STATE{Stop the iteration and exit the algorithm.}
	  \ENDIF
	  \STATE{Evaluate function value $r(x_k+d_k)$. 
	    Compute $\delta_k$ in~\eqref{def:pd} and $\rho_k$ in~\eqref{eqn:decrease-ratio-1}.}
		\STATE{Set $\theta_k$ in~\eqref{eqn:opt-ms-simp-bundle-merit} with $\theta_k = \max{\{\theta_{k-1},\eta_{\gamma}^- \norm{\lambda^{k+1}}_{\infty}+\gamma\}}$. If Algorithm~\ref{alg:simp-bundle-const} is called for iteration $k-1$, let $\theta_k = \max{\{\frac{1}{\pi_{k-1}},\eta_{\gamma}^- \norm{\lambda^{k+1}}_{\infty}+\gamma\}}$.}
	  \IF{$\rho_k > 0$}
		  \STATE{Find the line search parameter $\beta_k>0$ using backtracking, starting at $\beta_k=1$ and reducing by half 
		  if too large, such that the conditions in~\eqref{eqn:line-search-cond-alt} are satisfied.
		  Evaluate $r(x_{k+1})$ and compute $\rho_k^{\beta}$ in~\eqref{eqn:decrease-ratio-beta}.}
		  \IF{$\rho_k^{\beta} < 0$}
		    \STATE{Break and go to line 14.}
		  \ENDIF
		  \STATE{Take the step $x_{k+1} = x_k+\beta_k d_k$.}
	  \ELSE
		  \STATE{Reject the trial step.}
	    \STATE{Call the chosen $\alpha_k$ update rules to obtain $\alpha_{k+1}=\eta_{\alpha}\alpha_k$.}
	  \ENDIF
       \ENDFOR
    \end{algorithmic}
\end{algorithm}
%\subsection{Convergence analysis}
%Given the assumptions~\ref{}, first we list the properties necessary to prove convergence of the algorithm.
%\begin{lemma}\label{lem:properties}
%   Under the assumption made in Section, the following properties hold\\
%   (1) The sequence of solutions $x^k$ is bounded and the Lagrange function of the problem~\eqref{eqn:opt-ms} is lower bounded.\\ 
%	(2) There exists a constant $C_{\mu}>0$ such that for all sufficiently large $k$, we have 
%   \begin{equation}
%	   f_k+ r_{k,0} -(f_{k+1}+ r_{k+1,0}) \geq C_{\mu} \norm{x_{k+1}-x_k}^2
%   \end{equation}
%	(3) There exists $d_{k+1}\in \partial L_{x}(x_{k+1})$  such that 
%   \begin{equation}
%        \norm{d_{k+1}} \to 0, \text{as} \norm{x_{k+1}-x_k}  \to 0
%   \end{equation}
%	(4) The Lagrangian function $L(x)$ is continuous.
%\end{lemma}

%\begin{assumption}\label{assp:general}
%  The assumptions necessary to make the properties hold are\\
%  1 The feasible set for $x$ is bounded and the function $f(x)$ and $r(x)$ are continuous.\\
%  2 Function $r(x)$ is upper $C$-2.\\
%	3 For $\forall x \in X$, there exists subgradient for $r(x)$, denoted as $g(x) \in \partial_x r(x)$ \\
%\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Convergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Convergence analysis}\label{sec:alg-convg}
If the algorithm terminates in a finite number of steps, the stopping test at step 4 is satisfied with the error tolerance $\epsilon$ and the solution is considered found. 
Let $\epsilon=0$,  based on step 4, $\norm{d_k}= 0$.
Since $d_k$ solves~\eqref{eqn:opt-ms-simp-bundle}, optimality conditions in~\eqref{eqn:simp-bundle-KKT}
are satisfied, of which the first equation reduces to 
\begin{equation}\label{alg:finite-steps}
 \begin{aligned}
	 g_k- \nabla c(x_k) \lambda^{k+1}-\zeta_l^{k+1}+\zeta_u^{k+1}=0.
 \end{aligned}
\end{equation}
Given $g_k\in\bar{\partial} r(x_k)$, we have $0\in \bar{\partial} r(x_k)-\nabla c(x_k) \lambda^{k+1}-\zeta_l^{k+1}+\zeta_u^{k+1}$. 
In addition, by $c(x_k)+\nabla c(x_k)^T d_k = 0$ from~\eqref{eqn:simp-bundle-KKT}, we have $c(x_k)=0$. Thus, $x_k$ is feasible in terms of $c$. 
Since the bound constraints are enforced in the subproblem~\eqref{eqn:opt-ms-simp-bundle}, the rest of the equations in~\eqref{eqn:opt-ms-simp-KKT} are also satisfied.
Therefore,  $x_k$ satisfies~\eqref{eqn:opt-ms-simp-KKT} and is by definition a KKT point for~\eqref{eqn:opt-ms-simp} as the algorithm exits.
In what follows, the analysis is focused on the case with an infinite number of steps, \textit{i.e.}, $\norm{d_k}>0$. 
We start by showing that the parameter $\alpha_k$ in Algorithm~\ref{alg:simp-bundle} eventually stabilizes, \textit{i.e.}, becomes constant.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:sufficientdecrease}
	Given Assumption~\eqref{assp:upperC2}, Algorithm~\ref{alg:simp-bundle} produces a finite 
	number of rejected steps. 
	As a consequence, the quadratic coefficient $\alpha_k$  is bounded above and stays constant for $k$ large enough. 
\end{lemma}
\begin{proof}
%	At the $k$-th step of the algorithm, $x_{k+1}$ solves the subproblem~\eqref{eqn:opt-ms-simp-bundle}, hence
%\begin{equation} \label{eqn:opt-ms-appx-rec}
% \centering
%  \begin{aligned}
%	  r_k + g_{k}^T(x_{k+1}-x_k) + \frac{1}{2}\alpha_k \norm{x_{k+1}-x_k}^2 \leq r_{k},\\
%  \end{aligned}
%\end{equation}
%which implies
%\begin{equation} \label{eqn:opt-ms-appx-rec-2}
% \centering
%  \begin{aligned}
%	  g_{k}^T(x_{k+1}-x_k) + \frac{1}{2}\alpha_k \norm{x_{k+1}-x_k}^2 \leq 0.\\
%  \end{aligned}
%\end{equation}
	From the upper-$C^2$ inequality~\eqref{eqn:uppc2-def}, we have  
\begin{equation} \label{eqn:opt-ms-appx-rec-p1}
 \centering
  \begin{aligned}
	  r(x_k+d)- r_k - g_{k}^Td \leq C \norm{d}^2,\\
  \end{aligned}
\end{equation}
for a fixed constant $C>0$ on the bounded domain of $x$.
%	By summing~\eqref{eqn:opt-ms-appx-rec-2} and~\eqref{eqn:opt-ms-appx-rec-p1} we obtain
%\begin{equation} \label{eqn:opt-ms-appx-rec-p4}
% \centering
%  \begin{aligned}
%	  r_{k+1} + \frac{1}{2}\alpha_k \norm{x_{k+1}-x_k}^2 \leq C \norm{x_{k+1}-x_k}^2+r_{k}.\\
%  \end{aligned}
%\end{equation}
In the first part of the proof we show that if at some iteration $k$, $\alpha_k$ satisfies
\begin{equation} \label{eqn:opt-ms-appx-rec-p2}
 \centering
  \begin{aligned}
	  \alpha_k > 2 C, \\
  \end{aligned}
\end{equation}
then no rejected steps can occur in Algorithm~\ref{alg:simp-bundle} after iteration $k$, or equivalently, $\rho_t> 0$ and $\rho_t^\beta> 0$ for all iterations $t\geq k$.
%We remark that~\eqref{eqn:opt-ms-appx-rec-p4} implies that $r(\cdot)$ is reduced accordingly to 
%\begin{equation} \label{eqn:opt-ms-appx-rec-p3}
% \centering
%  \begin{aligned}%
%	  r_{k} -r_{k+1} \geq \tilde{\alpha}_0 \norm{x_{k+1}-x_k}^2.\\
%  \end{aligned}
%\end{equation}
The inequalities~\eqref{eqn:opt-ms-appx-rec-p1} and \eqref{eqn:opt-ms-appx-rec-p2} imply
\begin{equation} \label{eqn:opt-ms-appx-rec-obj}
 \centering
  \begin{aligned}
	  r_k - r(x_k+d_k) \geq& -g_{k}^T d_k -C \norm{d_k}^2\\
                        >& -g_{k}^T d_k -\frac{1}{2}\alpha_k \norm{d_k}^2
				 = \Phi_k(0) -\Phi_k(d_k). \\
  \end{aligned}
\end{equation}
	As in the definition~\eqref{eqn:decrease-ratio-1} of $\rho_k$, we distinguish between two cases based on the sign of $\delta_k$.
	If $\delta_k = \Phi_k(0) -\Phi_k(d_k) \geq 0$, then since $0<\eta_l^+\leq 1$,~\eqref{eqn:opt-ms-appx-rec-obj} gives  
\begin{equation} \label{eqn:opt-ms-appx-rec-obj2}
 \centering
  \begin{aligned}
	  r_k - r(x_k+d_k) >& \Phi_k(0) -\Phi_k(d_k) 
			\geq  \eta_l^+\left[ \Phi_k(0) -\Phi_k(d_k)\right]. 
  \end{aligned}
\end{equation}
If $\delta_k = \Phi_k(0) -\Phi_k(d_k) < 0$, given $\eta_l^-\geq 1$, we can also write based on~\eqref{eqn:opt-ms-appx-rec-obj} that  
\begin{equation} \label{eqn:opt-ms-appx-rec-obj3}
 \centering
  \begin{aligned}
	  r_k - r(x_k+d_k) >& \Phi_k(0) -\Phi_k(d_k) 
			\geq  \eta_l^-\left[ \Phi_k(0) -\Phi_k(d_k)\right]. 
  \end{aligned}
\end{equation}
As a consequence, by definition~\eqref{eqn:decrease-ratio-1} we conclude 
 $\rho_k > 0$. Similar inequalities hold for  $x_{k+1} = x_k+\beta_k d_k$ since one can write based on~\eqref{eqn:opt-ms-appx-rec-p1} that
\begin{equation} \label{eqn:opt-ms-appx-rec-merit-beta}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) \geq& -\beta_k g_{k}^Td_k - C \beta_k^2 \norm{d_k}^2 
                                 > -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2 \\
				 =& \Phi_k(0) -\Phi_k(\beta_k d_k).\\
  \end{aligned}
\end{equation}
Same reasoning that leads to~\eqref{eqn:opt-ms-appx-rec-obj2} and~\eqref{eqn:opt-ms-appx-rec-obj3} for $\eta_{\gamma}^+$ and $\eta_{\gamma}^-$ implies that  $\rho_k^{\beta}> 0$. Therefore, for all $t\geq k$, one has $\rho_t>0, \rho_t^{\beta}>0$ and thus $\alpha_t =\alpha_k$. 
%This completes the proof that no rejected steps occur once~\eqref{eqn:opt-ms-appx-rec-p2} holds.
Since Algorithm~\ref{alg:simp-bundle} increases $\alpha_k$ monotonically with a ratio $\eta_{\alpha}>1$ whenever a rejected step is encountered,
only a finite number of rejected steps are needed to reach $\alpha_k > 2 C$ and is followed by an infinite number of serious steps. 

For the second part of the proof, suppose now $\alpha_k \leq 2C$ for all $k$. 
This is only possible when no or a finite number of rejected steps have been taken by the algorithm followed by all serious steps. This completes the proof. 
%\begin{equation} \label{eqn:opt-ms-appx-ratio}
% \centering
%  \begin{aligned}
%       \rho_k \geq 1 \geq \eta_l.
%  \end{aligned}
%\end{equation}
%	Since $\alpha_k$ is increased when rejected steps happen,~\eqref{eqn:opt-ms-appx-rec-p2} will be %satisfied for $k$ large enough.
\end{proof}


\begin{remark}\label{rmrk:realalpha}
For simplicity, $\alpha_k$ is increased monotonically in the algorithm. In practice, we encourage that 
$\alpha_k$ be reduced if $\rho_k>0$ and $\eta_l^+>\eta_u^+$  where $\eta_u^+$ is an upper threshold for $\eta_l^+$.
In other words, if the actual decrease in objective is bigger than a certain ratio of the predicted decrease, 
	then $\Phi_k(\cdot)$ is a good approximation and we reduce the quadratic coefficient to encourage larger step size.
This adaptation is for when the upper-$C^2$ constant $C$ is not uniform in the entire domain. 
A decrease in $\alpha_k$ allows the algorithm to adjust better to  
	the local upper-$C^2$ constant that could be relatively small versus $C$, which could improve convergence.
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:line-search-merit}
	Given Assumption~\eqref{assp:boundedHc}, if the	Lagrange multipliers $\lambda^{k+1}$ of~\eqref{eqn:opt-ms-simp-bundle} is bounded, the line search process of Algorithm~\ref{alg:simp-bundle} is well-defined, in that 
	there exists $\beta_k\in (0, 1]$ that satisfies the line search conditions in~\eqref{eqn:line-search-cond-alt} and can be found in a finite number of steps through backtracking step 9 .
\end{lemma}
\begin{proof}
If $\lambda^{k+1}$ is bounded throughout the algorithm, then a finite and constant $\theta_k$ is guaranteed as well for $k$ large enough based on how it is chosen in Algorithm~\ref{alg:simp-bundle} step 7.
	%We show that there exists a $\beta_k>0$ independent of the line-search such that $\theta_k \norm{c(x_k)}_1 -\eta_{\gamma}^- \beta_k \left|(\lambda^{k+1})^T c(x_k)\right| \geq\theta_k \norm{c(x_{k+1})}_1-\eta_{\beta}\beta_k\frac{1}{2}\alpha_k\norm{d_k}^2$. 
	%In addition, the line search successfully terminates in a finite number of steps through backtracking, starting at $\beta_k=1$. 
	Since constraints $c$ are smooth, we apply Taylor expansion to the $j$th equality constraint, $j=1,\dots,m$, at $x_k$ for $x_{k+1}=x_k+\beta_k d_k$ to obtain 
   \begin{equation} \label{eqn:simp-bundle-c-ls-pf-1}
   \centering
    \begin{aligned}
	    c_j(x_{k+1})  = & c_j(x_k)+ \beta_k \nabla c_j(x_k)^T d_{k} + \frac{1}{2}\beta_k^2 d_k^T H_{k\beta}^{j} d_k,
   \end{aligned}
   \end{equation}
	where $H_{k\beta}^j$ is the Hessian $\nabla^2 c_j(\cdot)$ at a point on the line segment between $x_k$ and $x_{k+1}$. 
%   \begin{equation} \label{eqn:simp-bundle-c-taylor}
%   \centering
%    \begin{aligned}%
%	    c_j(x_{k+1}) - c_j(x_k)  = \nabla c_j(x_k)^T (x_{k+1}-x_{k})  + \frac{1}{2} d_k^T H_{k}^j d_k,\\
%    \end{aligned}
%   \end{equation}
%where $H_k^j$ is the Hessian $\nabla^2 c_j$ at a point on the line segment determined by $x_k$ and $x_{k+1}$.
Given $d_k$ as the solution to~\eqref{eqn:opt-ms-simp-bundle}, we have that $c_j(x_k) +  \nabla c_j(x_k)^T d_k = 0$ and, as a consequence, we can write based on~\eqref{eqn:simp-bundle-c-ls-pf-1} that
   \begin{equation*} %\label{eqn:simp-bundle-c-ls-pf-1}
    \centering
    \begin{aligned}
	    c_j(x_{k+1}) = (1-\beta_k) c_j(x_k)+ \frac{1}{2}\beta_k^2 d_k^T H_{k\beta}^{j} d_k.\\
    \end{aligned}
   \end{equation*}
By Assumption~\eqref{assp:boundedHc}, $\left|c_j(x_{k+1})\right|  \leq \left|(1-\beta_k) c_j(x_k)\right| + \beta_k^2 H^{c}_u \norm{d_k}^2$, which implies that
%   \begin{equation*} \label{eqn:simp-bundle-c-ls-pf-2}
%   \centering
%    \begin{aligned}
%	    \left|c_j(x_{k+1}^{\beta})\right|  =& \left|(1-\beta_k) c_j(x_k)+ \frac{1}{2}\beta_k^2 d_k^T H_{k\beta}^{j} d_k\right|
%	    \leq \left|(1-\beta_k) c_j(x_k)\right| + \beta_k^2 H^{c}_u \norm{d_k}^2,
%    \end{aligned}
%   \end{equation*}
%and, thus, one can write
   \begin{equation} \label{eqn:simp-bundle-c-ls-pf-2.5}
   \centering
    \begin{aligned}
	    \norm{c(x_{k+1})}_1  \leq 
	     (1-\beta_k) \norm{c(x_k)}_1 + m\beta_k^2 H^{c}_u \norm{d_k}^2.
    \end{aligned}
   \end{equation}
On the other hand, simple norm inequalities imply
\begin{equation} \label{eqn:simp-bundle-c-ls-pf-norm}
   \centering
    \begin{aligned}
	    \beta_k \left|(\lambda^{k+1})^T c(x_k)\right| \leq \beta_k\norm{\lambda^{k+1}}_{\infty} \norm{c(x_k)}_1.
    \end{aligned}
   \end{equation}
	Since step 7 of the algorithm chooses $\theta_k \geq \eta_{\gamma}^- \norm{\lambda^{k+1}}_{\infty}+\gamma$, where $\eta_{\gamma}^-$ and $\gamma$ are positive
	constants, we can write based on~\eqref{eqn:simp-bundle-c-ls-pf-2.5} and~\eqref{eqn:simp-bundle-c-ls-pf-norm} that
   \begin{equation} \label{eqn:simp-bundle-c-ls-pf-3} 
   \centering
    \begin{aligned}
	    &\theta_k\norm{c(x_k)}_1 -\eta_{\gamma}^- \beta_k \left|(\lambda^{k+1})^T c(x_k)\right|-\theta_k \norm{c(x_{k+1})}_1  \\ 
	    &\hspace{1.1cm}\geq(\theta_k - \eta_{\gamma}^- \beta_k\norm{\lambda^{k+1}}_{\infty}) \norm{c(x_k)}_1 -\theta_k(1-\beta_k) \norm{c(x_k)}_1 - \theta_km\beta_k^2 H^{c}_u \norm{d_k}^2\\
		&\hspace{1.1cm}=(\theta_k\beta_k- \eta_{\gamma}^- \beta_k\norm{\lambda^{k+1}}_{\infty}) \norm{c(x_k)}_1- \theta_km\beta_k^2 H^c_u  \norm{d_k}^2 \\
		&\hspace{1.1cm}\geq\beta_k \gamma \norm{c(x_k)}_1- \theta_k m \beta_k^2H^c_u\norm{d_k}^2.
    \end{aligned}
   \end{equation}
Therefore, if $\beta_k$ is reduced through the backtracking of Algorithm~\ref{alg:simp-bundle} to satisfy
   \begin{equation} \label{eqn:simp-bundle-c-ls-pf-4}
   \centering
    \begin{aligned}
	   0< \beta_k \leq \frac{\eta_{\beta} \alpha_k}{2 H^c_u\theta_k m},
    \end{aligned}
   \end{equation}
then~\eqref{eqn:line-search-cond-alt} is satisfied.
   %\begin{equation*} %\label{eqn:simp-bundle-c-ls-pf-5}
   %\centering
   % \begin{aligned}
%	    \theta_k \norm{c(x_k)}_1-\eta_{\gamma}^- \beta_k\left|(\lambda^{k+1})^T c(x_k)\right|-\theta_k \norm{c(x_{k+1})}_1 \geq  - \frac{1}{2}\eta_{\beta}\alpha_k\beta_k\norm{d_k}^2. 
%    \end{aligned}
%   \end{equation*}
Using ceiling function $\lceil\cdot \rceil$, which returns the least integer greater than the input, we can write 
   \begin{equation} \label{eqn:simp-bundle-c-ls-pf-5}
   \centering
    \begin{aligned}
	    \beta_k \geq \frac{1}{2} ^{\lceil \log_{\frac{1}{2}} \frac{\eta_{\beta} \alpha_k}{2 H^c_u\theta_k m} \rceil}.
    \end{aligned}
   \end{equation}
We remark that both the denominator and numerator in~\eqref{eqn:simp-bundle-c-ls-pf-4} are positive and independent of the line search. 
Further, by Lemma~\ref{lem:sufficientdecrease} and boundedness of $\lambda^{k+1}$, all terms in~\eqref{eqn:simp-bundle-c-ls-pf-4} remain finite. Therefore, the backtracking stops in finite steps.
%
%% do we need text below ?
%
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:line-search-alt}
	The $\beta_k \in (0,1]$ that meets the line search condition in~\eqref{eqn:line-search-cond-alt} also satisfies the conditions 
	from~\eqref{eqn:line-search-cond}, or equivalently
\begin{equation} \label{eqn:simp-bundle-etagamma}
   \centering
    \begin{aligned}
	   \beta_k(\lambda^{k+1})^T c(x_k)\geq -\theta_k \norm{c(x_k)}_1+ \theta_k \norm{c(x_{k+1})}_1 - \eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2,\\
	  \eta_{\gamma}^+\beta_k(\lambda^{k+1})^T c(x_k) \geq  -\theta_k \norm{c(x_k)}_1+ \theta_k \norm{c(x_{k+1})}_1   - \eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2,\\
	 \eta_{\gamma}^-\beta_k(\lambda^{k+1})^T c(x_k) \geq  -\theta_k \norm{c(x_k)}_1+ \theta_k \norm{c(x_{k+1})}_1 - \eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2.\\
    \end{aligned}
   \end{equation}
\end{lemma}
\begin{proof}
   From the absolute value inequality, we have  
   \begin{equation} \label{eqn:line-search-alt-pf-1}
   \centering
    \begin{aligned}
	    \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\beta_k\left|(\lambda^{k+1})^T c(x_k)\right|,\\ 
	     \eta_{\gamma}^+ \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\eta_{\gamma}^+ \beta_k\left|(\lambda^{k+1})^T c(x_k)\right|,\\
	     \eta_{\gamma}^- \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\eta_{\gamma}^-\beta_k\left|(\lambda^{k+1})^T c(x_k)\right|.\\
    \end{aligned}
   \end{equation}
	Given that $0<\eta_{\gamma}^{+}\leq 1\leq \eta_{\gamma}^-$, 
   \begin{equation} \label{eqn:line-search-alt-pf-2}
   \centering
    \begin{aligned}
            -\eta_{\gamma}^-\beta_k\left|(\lambda^{k+1})^T c(x_k)\right|\leq  -\beta_k\left|(\lambda^{k+1})^T c(x_k)\right| \leq -\eta_{\gamma}^+ \beta_k\left|(\lambda^{k+1})^T c(x_k)\right|.
    \end{aligned}
   \end{equation}
	Therefore, from~\eqref{eqn:line-search-alt-pf-1} and~\eqref{eqn:line-search-alt-pf-2}
   \begin{equation} \label{eqn:line-search-alt-pf-3}
   \centering
    \begin{aligned}
	    \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\eta_{\gamma}^- \beta_k\left|(\lambda^{k+1})^T c(x_k)\right|,\\ 
	     \eta_{\gamma}^+ \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\eta_{\gamma}^- \beta_k\left|(\lambda^{k+1})^T c(x_k)\right|,\\
	     \eta_{\gamma}^- \beta_k(\lambda^{k+1})^T c(x_k) \geq& -\eta_{\gamma}^-\beta_k\left|(\lambda^{k+1})^T c(x_k)\right|.\\
    \end{aligned}
   \end{equation}
   From the line search condition~\eqref{eqn:line-search-cond-alt}, we have
   \begin{equation} \label{eqn:line-search-alt-pf-4}
   \centering
    \begin{aligned}
	-\eta_{\gamma}^-\beta_k\left|(\lambda^{k+1})^T c(x_k)\right| \geq -\theta_k \norm{c(x_k)}_1+ \theta_k \norm{c(x_{k+1})}_1 - \eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2.\\
    \end{aligned}
   \end{equation}
   Combined with~\eqref{eqn:line-search-alt-pf-3} the proof is completed.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:sufficientdecrease-merit}
	The serious step $x_{k+1} = x_k+\beta_k d_k$ is a decreasing step for the merit function~\eqref{eqn:opt-ms-simp-bundle-merit} if $\beta_k$ is obtained via line search. Further, if $\lambda^k$ is bounded, the speed of decrease satisfies $\phi_{1\theta_k}(x_k)-\phi_{1\theta_k}(x_{k+1})>c_{\phi} \norm{d_k}^2$ for some $c_{\phi}>0$. 
\end{lemma}
\begin{proof}
	%We need to show that $\phi_{1k}(x_k) - \phi_{1k}(x_{k+1}) \geq 0$. 
	%By Lemma~\ref{lem:sufficientdecrease}, we know that there could only be finite number of rejected steps. 
	%Let $k$ be large enough so that all following steps are serious, and that $\alpha_t = \alpha_k$
	%for all $t>k$.
	For a serious step $x_{k+1}$ to be taken, step 8 and 10 are satisfied: $\rho_k>0,\rho_k^{\beta}>0$. 
	We distinguish three cases based on the value of $\alpha_k$ and sign of $\delta_k^{\beta}$. 
	The first case is $\alpha_k>2C$. By upper-$C^2$ property in~\eqref{eqn:opt-ms-appx-rec-p1}, as shown in~\eqref{eqn:opt-ms-appx-rec-merit-beta}, we have  
\begin{equation*} %\label{eqn:simp-bundle-merit-pf-1}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) >& -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2. \\
%				 =& \Phi_k(0) -\Phi_k(\beta_kd_k) = \delta_k^{\beta}.\\
  \end{aligned}
\end{equation*}
	%which leads to $\rho_k^{\beta}>0$.
	%which guarantees the decrease in the objective after line search. 
	In the second case, %the value $\alpha_k$ stabilizes 
	$\alpha_k\leq 2C$ and $\delta_k^{\beta}\geq 0 $.
	From the definition of $\rho_k^{\beta}$ in~\eqref{eqn:decrease-ratio-beta},  
\begin{equation} \label{eqn:simp-bundle-merit-pf-2p}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) > 
		  \eta_{\gamma}^+ \left[ -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2\right]. \\
  \end{aligned}
\end{equation}
       The third case is when $\alpha_k\leq 2C$ and $\delta_k^{\beta}<0$, and we have 
\begin{equation} \label{eqn:simp-bundle-merit-pf-2m}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) > 
		  \eta_{\gamma}^- \left[ -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2\right]. \\
  \end{aligned}
\end{equation}
%	Moreover, 
%\begin{equation} \label{eqn:simp-bunlde-merit-pf-2}
% \centering
%  \begin{aligned}
%	  \Phi_k(x_k) -\Phi_k(x_k+\beta_kd_k) =&-\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2\\
%	  \geq & -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k \norm{d_k}^2\\
%	  =& \beta_k \left[ \Phi_k(x_k) -\Phi_k(x_k+d_k)  \right]
%  \end{aligned}
%\end{equation}
		Rearranging the first equation in optimality conditions~\eqref{eqn:simp-bundle-KKT}, we have  
\begin{equation} \label{eqn:simp-bundle-KKT-beta}
  \centering
   \begin{aligned}
	   g_k + \alpha_k d_k =  \nabla c(x_k) \lambda^{k+1} +\zeta_l^{k+1} -\zeta_u^{k+1}.\\
   \end{aligned}
 \end{equation}
 By taking the inner product with $-d_k$ and using the last equation from~\eqref{eqn:simp-bundle-KKT}, we have 
\begin{equation} \label{eqn:simp-bundle-KKT-2}
  \centering
   \begin{aligned}
	   - g_k^T d_k-\alpha_k\norm{d_k}^2 &=- (\lambda^{k+1})^T \nabla c(x_k)^T d_k-d_k^T \zeta_l^{k+1}+d_k^T \zeta_u^{k+1}\\
			    &= (\lambda^{k+1})^T c(x_k) - (d_k - d_l^k +d_l^k)^T\zeta_l^{k+1} + (d_k-d_u^k+d_u^k)^T \zeta_u^{k+1} \\
			    &= (\lambda^{k+1})^T c(x_k) - (d_l^k)^T \zeta_l^{k+1}  +(d_u^k)^T \zeta_u^{k+1} \\
			    &= (\lambda^{k+1})^T c(x_k) + x_k^T \zeta_l^{k+1} + (x_u-x_k)^T\zeta_u^{k+1} \\
			    &\geq (\lambda^{k+1})^T c(x_k). \\
   \end{aligned}
 \end{equation}
	The third equality of~\eqref{eqn:simp-bundle-KKT-2} comes from $Z_{l}^{k+1}(d_k-d_l^k)=0$ and $Z_u^{k+1}(d_k-d_u^k)=0$ in~\eqref{eqn:simp-bundle-KKT}. 
	The inequality is obtained from bound constraints in~\eqref{eqn:simp-bundle-KKT-bound} 
	where $x_k\geq 0$, $x_u-x_k\geq 0$, $\zeta_l^{k+1}\geq 0$, and $\zeta_u^{k+1}\geq 0$
	for the current and previous iterations. 
	Next, multiplying both sides of~\eqref{eqn:simp-bundle-KKT-2} by $\beta_k$ and then subtracting $\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2$ leads to
  \begin{equation} \label{eqn:simp-bundle-KKT-3}
       \centering
       \begin{aligned}
	       -\beta_kg_k^T d_k-\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2 &\geq \alpha_k\beta_k\norm{d_k}^2-\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2+\beta_k(\lambda^{k+1})^Tc(x_k)\\
		 &\geq\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2+\beta_k(\lambda^{k+1})^Tc(x_k),\\
         \end{aligned}
        \end{equation}
	where the second inequality makes use of $\beta_k\in (0,1]$.
Notice that the left-hand side of~\eqref{eqn:simp-bundle-KKT-3} is $\delta_k^{\beta}$. 
Multiplying both sides of~\eqref{eqn:simp-bundle-KKT-3} by $\eta_{\gamma}^+$ and $\eta_{\gamma}^-$ respectively, we obtain
  \begin{equation} \label{eqn:simp-bundle-KKT-4}
       \centering
       \begin{aligned}
	       -\eta_{\gamma}^+ \beta_kg_k^T d_k-\frac{1}{2}\eta_{\gamma}^+\alpha_k\beta_k^2\norm{d_k}^2 
	       %&\geq \eta_{\beta}\alpha_k\beta_k\norm{d_k}^2-\frac{1}{2}\eta_{\beta}\alpha_k\beta_k^2\norm{d_k}^2+\eta_{\beta}\beta_k(\lambda^{k+1})^Tc_k\\
		 &\geq\frac{1}{2}\eta_{\gamma}^+\alpha_k\beta_k\norm{d_k}^2+\eta_{\gamma}^+\beta_k(\lambda^{k+1})^Tc(x_k),\\
         \end{aligned}
        \end{equation}
  \begin{equation} \label{eqn:simp-bundle-KKT-5}
       \centering
       \begin{aligned}
	       -\eta_{\gamma}^- \beta_kg_k^T d_k-\frac{1}{2}\eta_{\gamma}^-\alpha_k\beta_k^2\norm{d_k}^2 
		 &\geq\frac{1}{2}\eta_{\gamma}^-\alpha_k\beta_k\norm{d_k}^2+\eta_{\gamma}^-\beta_k(\lambda^{k+1})^Tc(x_k).\\
         \end{aligned}
        \end{equation}
Finally, we examine the merit function $\phi_{1\theta_k}(\cdot)$. If $\alpha_k>2C$, 
we combine the inequality in~\eqref{eqn:opt-ms-appx-rec-merit-beta},~\eqref{eqn:simp-bundle-KKT-3}, and the first inequality from Lemma~\ref{lem:line-search-alt} to write
\begin{equation} \label{eqn:simp-bundle-merit-pf-3}
 \centering
  \begin{aligned}
	  \phi_{1\theta_k}(x_k) - \phi_{1\theta_k}(x_{k+1})  &= r(x_k) -r(x_{k+1})+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 >& -\beta_kg_k^T d_k-\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1 \\
			 \geq&\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2+\beta_k(\lambda^{k+1})^Tc(x_k)+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 \geq&\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2-\eta_{\beta}\beta_k\frac{1}{2}\alpha_k\norm{d_k}^2
			 = (1-\eta_{\beta})\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2.
  \end{aligned}
\end{equation}
Similarly, if $\alpha_k\leq 2C$ and $\delta_k^{\beta}\geq 0$, by applying in order~\eqref{eqn:simp-bundle-merit-pf-2p},~\eqref{eqn:simp-bundle-KKT-4} and the second inequality from Lemma~\ref{lem:line-search-alt}, we write 
\begin{equation} \label{eqn:simp-bundle-merit-pf-4}
 \centering
  \begin{aligned}
	  \phi_{1\theta_k}(x_k) - \phi_{1\theta_k}&(x_{k+1})  = r(x_k) -r(x_{k+1})+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 >& -\eta_{\gamma}^+\beta_kg_k^T d_k-\eta_{\gamma}^+\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1 \\
			 \geq&\frac{1}{2}\eta_{\gamma}^+\alpha_k\beta_k\norm{d_k}^2+\eta_{\gamma}^+\beta_k(\lambda^{k+1})^Tc(x_k)+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 \geq&\frac{1}{2}\eta_{\gamma}^+\alpha_k\beta_k\norm{d_k}^2-\eta_{\beta}\beta_k\frac{1}{2}\alpha_k\norm{d_k}^2
			 = (\eta_{\gamma}^+-\eta_{\beta})\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2.
  \end{aligned}
\end{equation}
Recall that $\eta_{\gamma}^+-\eta_{\beta}>0$ by design of Algorithm~\ref{alg:simp-bundle}. Finally, when $\delta_k^{\beta}\leq 0$, applying
in order~\eqref{eqn:simp-bundle-merit-pf-2m},~\eqref{eqn:simp-bundle-KKT-5} and the third inequality from Lemma~\ref{lem:line-search-alt}, we have 
\begin{equation} \label{eqn:simp-bundle-merit-pf-5}
 \centering
  \begin{aligned}
	  \phi_{1\theta_k}(x_k) - \phi_{1\theta_k}&(x_{k+1})  =r(x_k) -r(x_{k+1}^{\beta})+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 >& -\eta_{\gamma}^-\beta_kg_k^T d_k-\eta_{\gamma}^-\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1 \\
			 \geq&\frac{1}{2}\eta_{\gamma}^-\alpha_k\beta_k\norm{d_k}^2+\eta_{\gamma}^-\beta_k(\lambda^{k+1})^Tc(x_k)+\theta_k\norm{c(x_k)}_1-\theta_k\norm{c(x_{k+1})}_1\\
			 \geq&\frac{1}{2}\eta_{\gamma}^-\alpha_k\beta_k\norm{d_k}^2-\eta_{\beta}\beta_k\frac{1}{2}\alpha_k\norm{d_k}^2
			 = (\eta_{\gamma}^- -\eta_{\beta})\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2,
  \end{aligned}
\end{equation}
where $\eta_{\gamma}^- -\eta_{\beta}>0$.
Therefore, in all cases, a serious step $x_{k+1}=x_k+\beta_kd_k$ is a 
decreasing direction for $\phi_{1\theta_k}(\cdot)$. 
%From Lemma~\ref{lem:line-search-alt}, line search is completed as soon as $\beta_k$ satisfies~\eqref{eqn:simp-bundle-c-ls-pf-4}. 
If $\lambda^{k}$ is bounded, $\theta_k$ will stay constant for $k$ large enough from step 7 of Algorithm~\ref{alg:simp-bundle}. Let $\bar{\theta}$ be the constant value so that $\theta_k \leq \bar{\theta}$ for all $k$.  
Then, by~\eqref{eqn:simp-bundle-c-ls-pf-5},
\begin{equation} \label{eqn:simp-bundle-merit-pf-6}
 \centering
  \begin{aligned}
	  \beta_k \geq \frac{1}{2} ^{\lceil \log_{\frac{1}{2}} \frac{\eta_{\beta} \alpha_0}{2 H^c_u\bar{\theta} m} \rceil}:=\bar{\beta},
  \end{aligned}
\end{equation}
due to the monotonicity of $\alpha_k$ and $\theta_k$. In other words, $\beta_k$ is bounded below by $\bar{\beta}$ for all $k$.
From~\eqref{eqn:simp-bundle-merit-pf-3},~\eqref{eqn:simp-bundle-merit-pf-4},~\eqref{eqn:simp-bundle-merit-pf-5}, $\phi_{1\theta_k}(x_k)-\phi_{1\theta_k}(x_{k+1})>(\eta_{\gamma}^+-\eta_{\beta})\frac{1}{2}\alpha_0 \bar{\beta}\norm{d_k}^2$. 
Or simply, there exists $c_{\phi}>0$ such that $\phi_{1\theta_k}(x_k)-\phi_{1\theta_k}(x_{k+1})>c_{\phi}\norm{d_k}^2$. 
\end{proof}
%\begin{lemma}\label{lem:bounded}
%  $x$  is bounded and the Lagrangian function of~\eqref{eqn:opt-fcn} is 
%  continuous bounded below.
%\end{lemma}
In order to attain bounded Lagrange multipliers, a constraint qualification is necessary 
for $c$ in~\eqref{eqn:opt-ms-simp}.
%This is an area 
%beyond the scope of this work and at the same time has enjoyed
%rich research. 
%In Section~\ref{sec:prob}, we discussed calmness as the weak constraint qualification that 
%would ensure a KKT point instead of a Fritz-John critical point for~\eqref{eqn:opt-ms-simp}.
Given the existence of both equality and inequality constraints, we resort to LICQ~\cite{Nocedal_book}. A topic of further research will be to obtain global convergence under a weaker constraint qualification such as the Slater condition. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:bounded-lp}
	If LICQ of the constraints in~\eqref{eqn:opt-ms-simp} are satisfied at every accumulation points $\bar{x}$ of serious steps $\{x_k\}$ generated by the algorithm, then 
	the sequence of Lagrange multipliers for problem~\eqref{eqn:opt-ms-simp-bundle} $\{\zeta_u^{k+1}\},\{\zeta_l^{k+1}\}$ and $\{\lambda^{k+1}\}$ are bounded. 
	%Thus, there exists $k$, such that $\norm{\lambda^{t}}_{\infty} \leq \lambda^U$, $\zeta^{t}_u \leq \zeta_u^U$ and $\zeta^{t}_l \leq \zeta_l^U$ for all $t\geq k$, where $\lambda^U>0,\zeta_u^U>0,\zeta_l^U>0$ are the upper bounds. 
	Further, this means there exists $k$ such that $\theta_t = \theta_k$ for all $t\geq k$.
\end{lemma}
\begin{proof}
     We rewrite the first equation in optimality condition in~\eqref{eqn:simp-bundle-KKT} as
    \begin{equation} \label{eqn:simp-bundle-KKT-full}
     \centering
     \begin{aligned}
	     g_k + \alpha_k d_k - \sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k) -\sum_{i=1}^n (\zeta_l^{k+1})_i e_i 
	     +\sum_{i=1}^n (\zeta_u^{k+1})_i e_i &=0,\\
     \end{aligned}
    \end{equation}
    where $e_i \in \Rbb^n$ is a vector such that $(e_i)_i = 1$ and $(e_i)_l = 0,l\neq i$. 
    The Lagrange multipliers for the bound constraints can be combined into one vector $\zeta^{k+1}=\zeta_l^{k+1}- \zeta_u^{k+1}$,
    since $(\zeta_l^{k+1})_i(\zeta_u^{k+1})_i = 0$.
	A component of $\zeta_l^{k+1}$ or $\zeta_u^{k+1}$ is unbounded if and only if the corresponding component in $\zeta^{k+1}$ is unbounded.
	Let $I$ be the index set of the active bound constraints, we have
    \begin{equation} \label{eqn:simp-bundle-KKT-full-2}
     \centering
     \begin{aligned}
	     g_k + \alpha_k d_k = \sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k) +\sum_{i \in I} (\zeta^{k+1})_i e_i.\\
     \end{aligned}
    \end{equation}
	Since $\{x_k\},\{g_k\}$ are bounded ($r$ being Lipschitz on a bounded domain) and $\{\alpha_k\}$ is finite by Lemma~\ref{lem:sufficientdecrease}, 
	the left-hand side of the equation stays bounded as $k\to\infty$. 
	From LICQ at $\bar{x}$, $\nabla c_j(\bar{x}) \in \Rbb^n $ and $e_i,i \in I$ are linearly independent and bounded vectors. 
	Without losing generality, suppose $\lambda^{k+1}_j,j\in[1,m]$ is not 
	bounded as $k\to\infty$. Then, $\norm{\lambda^{k}}_{\infty} \to \infty$ and we can construct an unbounded subsequence $\{\lambda^{k_u}\}$ that is monotonic in $\lambda^{k_u}_j$. The corresponding subsequences $\{x_{k_u}\}$, $\{g_{k_u}\}$, $\{\alpha_{k_u}\}$ remain bounded. Passing on further to a subsequence if necessary, in which case the subsequence of $\{\lambda^{k_u}\}$ is still unbounded, we can assume $x_{k_u}\to\bar{x}$ as $k\to\infty$, where $\bar{x}$ is an accumulation point. Regardless of the behavior of $\{\zeta^{k_u}\}$, the right-hand side of~\eqref{eqn:simp-bundle-KKT-full-2} will be unbounded due to linear independence at $\bar{x}$ among the vectors.
	This is a contradiction. Same process can be repeated for $\zeta^{k+1}_j,j\in[1,m]$. 
	Therefore, there exist $\lambda^U\geq 0$, $\zeta_l^U\geq 0$, $\zeta_u^U\geq 0$  such that 
	$\norm{\lambda^{k}}_{\infty} \leq \lambda^U$, $\zeta^{k}_u \leq \zeta_u^U$ and $\zeta^{k}_l \leq \zeta_l^U$ for all $k$.
	Since $\theta_k$ is determined by $\lambda^k$, there exists $k$ such that $\theta_t=\theta_k$ for all $t\geq k$. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:simp-KKT}
	Given the Assumptions~\eqref{assp:upperC2} and~\eqref{assp:boundedHc}, if the constraints in~\eqref{eqn:opt-ms-simp} satisfy the 
	conditions in Lemma~\ref{lem:bounded-lp}, then every accumulation point $\bar{x}$ of the serious steps $\{x_k\}$ generated by Algorithm~\ref{alg:simp-bundle} 
	is a KKT point of the problem~\eqref{eqn:opt-ms-simp}. 
	That is, there exists a subsequence $\{x_{k_s}\}$ of $\{x_k\}$, where $ x_{k_s} \to \bar{x}$, and $\bar{\lambda}\in\Rbb^m$, $\bar{\zeta}_u\in\Rbb^n$, $\bar{\zeta}_l\in\Rbb^n$, so that the first-order optimality conditions~\eqref{eqn:opt-ms-simp-KKT} are satisfied at $\bar{x}$.
%\begin{equation} \label{eqn:simp-bundle-KKT-limit}
% \centering
%  \begin{aligned}
%	  0 \in \bar{\partial} r(\bar{x}) - \nabla c(\bar{x}) \bar{\lambda}-\bar{\zeta}_l +\bar{\zeta}_u&, \\
%	  \bar{Z}_l\bar{x} = 0,\  \bar{Z}_u(\bar{x}-x_u) = 0&,\\
%	  c(\bar{x}) = 0&,\\
%	  \bar{\zeta}_l,\bar{\zeta}_u,\bar{x}, x_u-\bar{x} \geq 0&.\\
%  \end{aligned}
%\end{equation}
\end{theorem}
\begin{proof}
	By Lemma~\ref{lem:sufficientdecrease}, there exists $k_0>0$ such that for all $t\geq k_0$, $\alpha_t=\alpha_{k_0}=\bar{\alpha}$ and 
	all steps are serious steps.
	%Therefore, the ratio for the objective satisfies the serious step test as  
	%$\rho_k > 0$ and $\rho_k^{\beta}>0$.
	By Lemma~\ref{lem:bounded-lp}, there exists $k_1>0$ such that for $t\geq k_1$, the Lagrange multipliers are bounded above and $\theta_t=\theta_{k_1}=\bar{\theta}$. 
	We say $k$ is large enough if $k\geq \max{(k_0,k_1)}$, in which case the parameters of the algorithm stabilizes at $\alpha_t=\bar{\alpha}$ and $\theta_t=\bar{\theta}$ for $t\geq k$.

	Since the domain of $x$ is bounded and $r$ is Lipschitz, the serious steps sequence $\{x_k\}$ 
	as well as the subgradient sequence $\{g_{k}\}$ are bounded. 
	Therefore, there exists at least one accumulation point for $\{x_k\}$.
	Let $\bar{x}$ be an accumulation point of $\{x_k\}$ and $\{x_{k_s}\}$ be a subsequence of $\{x_k\}$ such that $x_{k_s}\to \bar{x}$.

	From Lemma~\ref{lem:line-search-merit}, line search terminates successfully and  
	by Lemma~\ref{lem:sufficientdecrease-merit}, for $k$ large enough, $\{\phi_{1\theta_k}(x_k)\}$ is a decreasing and bounded sequence 
	with a fixed parameter $\bar{\theta}$. 
	Thus, $\phi_{1\theta_k}(x_k)$ converges. 
	%Let $\lim_{k\to\infty} \phi_{1k}(x_k)\to \bar{\phi}_{1k}$, or equivalently $\lim_{k\to\infty}r(x_k)+\bar{\theta}\norm{c(x_k)}_1 \to \bar{\phi}_{1k}$. 
	From Lemma~\ref{lem:sufficientdecrease-merit},
	%~\eqref{eqn:simp-bundle-merit-pf-3},~\eqref{eqn:simp-bundle-merit-pf-4} and~\eqref{eqn:simp-bundle-merit-pf-5}, 
	we know that $\phi_{1\theta_k}(x_k)-\phi_{1\theta_k}(x_{k+1})$ is 
	bounded below in the order of $\norm{d_k}^2$. Therefore,  $\lim_{k\to\infty} \norm{d_k}\to 0$. In particular, $\lim_{s\to \infty}\norm{d_{k_s}}\to 0$.
	By the last equation in~\eqref{eqn:simp-bundle-KKT}, $c(x_{k_s})\to 0$. Thus, $\bar{x}$ satisfies the equality constraints $c$.
        Given that the bound constraints are satisfied by all $x_k$, we have $0\leq \bar{x}\leq x_u$. 
          
	Passing on to a subsequence if necessary, we let $g_{k_s}\to \bar{g}$, 
	$\lambda^{k_{s}+1} \to \bar{\lambda}$, $\zeta_u^{k_{s}+1} \to \bar{\zeta}_u$, $\zeta_l^{k_{s}+1} \to \bar{\zeta}_l$. 
        From the first equation in the optimality conditions~\eqref{eqn:simp-bundle-KKT}, we have 
        \begin{equation} \label{eqn:simp-bundle-KKT-limit-1}
          \centering
          \begin{aligned}
		  0 = \bar{g} - \nabla c(\bar{x}) \bar{\lambda}  -\bar{\zeta}_l +\bar{\zeta}_u. 
          \end{aligned}
        \end{equation}
	%Notice that $x_{k}+d_k$ (not $x_{k+1}$) solves~\eqref{eqn:opt-ms-simp-bundle} at $x_k$. Therefore, at the accumulation point, 
	%$\bar{x}$ solves~\eqref{eqn:opt-ms-simp-bundle} at $x_k=\bar{x}$, or $\bar{d}=0$. The optimality condition at $x_k=\bar{x}$ means 
	By the outer semicontinuity of Clarke subdifferential, with $g_{k_s}\in \bar{\partial} r(x_{k_s})$, we have $\bar{g} \in \bar{\partial} r(\bar{x})$.
        As a result, 
	  $0 \in \bar{\partial} r(\bar{x}) -\nabla c(\bar{x}) \bar{\lambda} -\bar{\zeta}_l +\bar{\zeta}_u$.
	The complementarity conditions of bound constraints from~\eqref{eqn:simp-bundle-KKT} lead 
	to $\bar{Z}_u(\bar{x}-x_u)$, $\bar{Z}_l\bar{x}=0$. Together with the 
	equality constraints $c(\bar{x}) = 0$, the first-order necessary 
	optimality conditions~\eqref{eqn:opt-ms-simp-KKT} of problem~\eqref{eqn:opt-ms-simp} at $\bar{x}$ are satisfied.
	%By the first-order optimality condition, $g^*= \lim_{k\to\infty} \lambda^{k}+\zeta^k\nabla c_k$.
	%Given that sequences $\{\alpha_k\}$,$\{\zeta^k\}$, $\{\lambda_k\}$ are bounded, 
 %Passing on further to a subsequence if necessary, let $\lambda^*$ be the subsequent limit of $\{\lambda^k\}$, 
%	then $\lambda^*=\lim_{k\to\infty}\lambda^{k}\geq 0$. If $\nabla c^*\neq 0$, then $\lim_{k\to\infty}\zeta_k = \frac{g^*-\lambda^*}{\nabla c^*}$.
%	Otherwise, $\zeta^*$ can be chosen to be any finite real scalar.
%	So, there exist $\lambda^*,\zeta^*$, which together with $g^*$ and $x^*$ satisfy the first-order optimality conditions, or KKT condition in~\eqref{eqn:simp-bundle-KKT-limit}, making $x^*$ a KKT point.
\end{proof}

%\begin{proposition}\label{prop:subgradient}
%	If function $r(x)$ is continuously differentiable, then  
%	the subgradient of the Lagrangian function of the full problem $d_{k+1} \in \partial_x L(x_{k+1})$ satisfies (2) in Lemma~\ref{lem:properties}.
%	In addition, every accumulation point of $x_k$ is a KKT point.
%\end{proposition}
%\begin{proof}
%Let $g_{k+1} \in \partial r(x_{k+1})$, and 

%\begin{equation} \label{eqn:opt-ms-appx-rec-p3}
% \centering
%  \begin{aligned}
%	  0 &= \pder{L_k}{x}(x_{k+1})=  g_{k} + \alpha_k(x_{k+1}-x_k) - \lambda_{k+1}^Tc(x_{k+1}),\\
%  \end{aligned}
%\end{equation}
%where $\lambda$ is the Lagrange multiplier for the corresponding remaining constraints and bounds,
%denoted as $z(x)$. The underscore in the Lagrange function $L$ indicates that it is the full problem
%with quadratic recourse approximation, and thus continuously differentiable.
%The real subgradient $\partial_x L(x_{k+1})$ with the same Lagrange multipliers on the other hand is given by
%\begin{equation} \label{eqn:opt-ms-appx-rec-p3}
% \centering
%  \begin{aligned}
%   \partial_x L (x_{k+1})=g_{k+1} - \lambda_{k+1}^Tz_{k+1}\\
%  \end{aligned}
%\end{equation}
%Thus we have 
%\begin{equation} \label{eqn:opt-ms-appx-rec-p3}
% \centering
%  \begin{aligned}
%	  \norm{d_{k+1}} = \norm{\partial_x L (x_{k+1})}&=\norm{ g_{k+1} - g_{k}}-\alpha_k\norm{x_{k+1}-x_k}\\
%	  &= \norm{g_{k+1}-g_k}+\alpha_k\norm{x_{k+1}-x_k}
%  \end{aligned}
%\end{equation}
%	Since $r(x)$ is continuously differentiable, we have 
%	$\norm{g_{k+1}-g_k}\to 0$, as $\norm{x_{k+1}-x_k} \to 0$.
%Hence,
%\begin{equation} \label{eqn:opt-ms-appx-rec-p3}
% \centering
%  \begin{aligned}
%	  \norm{d_{k+1}} \to 0,\norm{x_{k+1}-x_k} \to 0.
%  \end{aligned}
%\end{equation}

%	From Theorem~\ref{thm:simp-KKT}, we know that there exist sequences produced by the algorithm $x_{k_p}\to \bar{x}$ as
%	$k_p\to\infty$. Therefore, $\{d_{k_p}\}\to 0$. The argument for the existence of $\lambda^*$ is the same as in the proof
%	of Theorem~\ref{thm:simp-KKT}. Therefore, every accumulation point of $x_{k_p}$ is a KKT point.
%\end{proof}
While the line search is only conducted on the less computationally expensive and analytically known 
smooth constraints $c$, it is 
possible to avoid it altogether. In bundle methods, it has been shown that a convex feasible set for $x$ can make the 
algorithm converge without line search~\cite{hare2015}. Similarly, if the constraints form a convex feasible set, 
we have the following result for the simplified bundle algorithm.  
\begin{proposition}\label{prop:convex-constraint}
	If the equality constraint $c$ and bound constraints in~\eqref{eqn:opt-ms-simp} form a convex and bounded set in $\Rbb^n$, 
	then instead of~\eqref{eqn:opt-ms-simp-bundle} we solve subproblem
        \begin{equation} \label{eqn:opt-ms-simp-bundle-2}
        \centering
         \begin{aligned}
          &\underset{\substack{x}}{\text{minimize}} 
	  & & \phi_k(x)\\
          &\text{subject to}
	  & & c(x) = 0, ~0 \leq x\leq x_u.
  \end{aligned}
\end{equation}
	And the line search step can be skipped with $x_{k+1} = x_k +d_k$, $d_k$ being the solution to~\eqref{eqn:opt-ms-simp-bundle-2}.
	The global convergence is maintained.
\end{proposition}

%Using the subgradient 
%\begin{equation} \label{eqn:opt-rc-mu-simp-p1}
%\centering
% \begin{aligned}
%	 r_{i,\mu}(x_2)-&r_{i,\mu}(x_1)- g_1(x_2-x_1) \\
%	 =& p_{i,\mu}(x_2,y_2)-p_{i,\mu}(x_1,y_1)-\pder{p_{i,\mu}}{x}^T(x_1,y_1)(x_2-x_1)\\
%	 =& d_i\mu |Wx_2 - g(y_2)|^2 - d_i\mu |Wx_1 - g(y_1)|^2 - 2d_i\mu (Wx_1 - g(y_1))^TW(x_2-x_1)\\
%	 =& d_i\mu (x_2^T W^T W x_2 -2g(y_2)^TWx_2 +g(y_2)^Tg(y_2))\\& - d_i\mu (x_1^T W^T W x_1 -2g(y_1)^TWx_1 +g(y_1)^Tg(y_1))\\
%	  &  - 2d_i\mu  (x_1^TW^TWx_2- x_1^TW^TWx_1-g(y_1)^TWx_2+g(y_1)^TWx_1  )\\
%	 =& d_i\mu( |Wx_2-Wx_1|^2 -2g(y_2)^TWx_2 +g(y_2)^Tg(y_2)  -g(y_1)^Tg(y_1)\\
%	  &          +2g(y_1)^TWx_2 )
% \end{aligned}
%\end{equation}
%Let $x_2-x_1=hd, |d|=1$, one way of simplifying the above equation gets us
%On the other hand,
%\begin{equation} \label{eqn:opt-rc-mu-simp-p3}
%\centering
% \begin{aligned}
%	 r_{i,\mu}(x_2)-r_{i,\mu}(x_1)- &g_1(x_2-x_1) \\
%	 =& d_i\mu( |Wx_2-Wx_1|^2 -2g(y_2)^TWx_2 +g(y_2)^Tg(y_2)  -g(y_1)^Tg(y_1)\\
%	  &          +2g(y_1)^TWx_2 )\\
%	 =& d_i\mu( h^2|Wd|^2 +|g(y_2) - Wx_1|^2+2g(y_2)^TWx_1-|g(y_1) - Wx_1|^2\\
%	  &          -2g(y_1)^TWx_1 -2g(y_2)^TWx_2 +2g(y_1)^TWx_2 )\\
%	 =& d_i\mu( h^2|Wd|^2 +|g(y_2) - Wx_1|^2-|g(y_1) - Wx_1|^2\\
%	  &          -2g(y_1)^T(Wx_1-Wx_2) +2g(y_2)^T(Wx_1-Wx_2) )\\
%	 \geq& d_i\mu( h^2|Wd|^2 -2g(y_1)^T(Wx_1-Wx_2) +2g(y_2)^T(Wx_1-Wx_2) )\\
%	 =& d_i\mu( h^2|Wd|^2 -2h[g(y_1)-g(y_2)]^TWd )\\
% \end{aligned}
%\end{equation}

%Another way of looking at the equation is 
%\begin{equation} \label{eqn:opt-rc-mu-simp-p4}
%\centering
% \begin{aligned}
%	 &d_i\mu\{ h^2|Wd|^2 -2(g(y_2)-g(y_1))^TWx_2 +(g(y_2))+g(y_1))^T(g(y_2)-g(y_1)) \}\\
%	 &=d_i\mu\{ h^2|Wd|^2- (g(y_2)-g(y_1))^T (2Wx_2 - g(y_2)-g(y_1)) \}\\
%	 &=d_i\mu\{ h^2|Wd|^2- (g(y_2)-g(y_1))^T (Wx_2 - g(y_2) +Wx_1-g(y_1) +hd) \}\\
% \end{aligned}
%\end{equation}

%A major assumption needs to be made on $|g(y_2)-g(y_1)|<Gh$

%\begin{equation} \label{eqn:opt-rc-mu-simp-p5}
%\centering
% \begin{aligned}
%	 &d_i\mu\{ h^2|Wd|^2- (g(y_2)-g(y_1))^T (Wx_2 - g(y_2) +Wx_1-g(y_1) +hd) \}\\
%	 &\leq d_i\mu\{ h^2|Wd|^2 +Ch^2- (g(y_2)-g(y_1))^T(Wx_2 - g(y_2) +Wx_1-g(y_1) ) \}\\
%	 &= d_i\mu\{ ch^2- (g(y_2)-g(y_1))^T(Wx_2 - g(y_2))- (g(y_2)-g(y_1))^T (Wx_1-g(y_1) ) \}\\
%	 &= d_i\mu\{ ch^2 + (\nabla g(y_2)^T(y_1-y_2)+k_1|y_1-y_2|^2)^T(Wx_2 - g(y_2))\\\quad&- 
%	    (\nabla g(y_1)^T(y_2-y_1)+k_2|y_1-y_2|^2)^T (Wx_1-g(y_1) ) \}\\   
% \end{aligned}
%\end{equation}


%Taking a closer look at the linear part
%\begin{equation} \label{eqn:opt-rc-mu-simp-p6}
%\centering
% \begin{aligned}
%	 &  (\nabla g(y_2)^T(y_1-y_2))^T(Wx_2 - g(y_2))- 
%	    (\nabla g(y_1)^T(y_2-y_1))^T (Wx_1-g(y_1)) \\
%	 & = (y_1-y_2)^T \nabla g(y_2)(Wx_2 - g(y_2))- 
%	    (y_2-y_1)^T \nabla g(y_1)(Wx_1-g(y_1)) \\
%	 & = (y_1-y_2)^T [\nabla g(y_2)(Wx_2 - g(y_2)) + \nabla g(y_1)(Wx_1-g(y_1))]\\
% \end{aligned}
%\end{equation}
%The optimality condition gives
%\begin{equation} \label{eqn:opt-rc-mu-simp-p7}
%\centering
% \begin{aligned}
%	 \nabla g(y_2)(Wx_2 - g(y_2)) + \lambda_1 \text{(for c)} - \lambda_2 \text{(for d)}  = 0\\
%	 \nabla g(y_2)(Wx_2 - g(y_2)) = \lambda\\
% \end{aligned}
%\end{equation}

%\subsection{Application to two-stage stochastic optimization problem}\label{sec:app}
The algorithm and convergence analysis can be readily extended to two-stage stochastic programming problems in the form of 
~\eqref{eqn:opt0}, 
where the quadratic approximation function $\phi_k(\cdot)$ is needed only for second-stage solution function $r$. Details of the setup and additional update rules for $\alpha_k$
can be found in the report~\cite{wang2022}.

%Problem~\eqref{eqn:opt-ms} is approximated locally as 
%\begin{equation} \label{eqn:opt-ms-phi}
% \centering
%  \begin{aligned}
%   &\underset{\substack{x\in \Rbb^n}}{\text{min}} 
%	  & & f(x)+ \phi_k(x)\\
%   &\text{s.t.}
%	  & & c(x) =c_E\\
%	  &&& d^l \leq d(x) \leq d^u\\
%	  &&& x^l \leq x \leq x^u,\\
%  \end{aligned}
%\end{equation}
%if $r_i$ is Lipschitz and upper-$C^2$. 
%The first-stage objective $f(\cdot)$, which is twice continuously differentiable, 
%is kept as it is. As a result, we can take advantage of the sparsity structure arising
%from first-stage problems as the Hessian of $\phi_k(\cdot)$ is diagonal.
%
%The update rule of $\alpha_k$ is critical and problem dependent. 
%It is a trade-off between robust convergence behavior (large $\alpha_k$) and fast but potentially unstable convergence (small $\alpha_k$). The $\alpha_k$ in Algorithm~\ref{alg:simp-bundle} does not 
%bear much meaningful structure from the objective function since the Hessian itself might not exist. 
%Nevertheless, for many problems with more differentiability, it is 
%possible to explore ways to extract more second-order information.

%One update option is to use the Barzilai-Borwein (BB) gradient method~\cite{barzilai_1988}, 
%which can be interpreted as an approximation to the secant equation. The update rule for $\alpha_k$ is
%\begin{equation} \label{eqn:alpha-BB}
% \centering
%  \begin{aligned}
%	  \alpha_k = \frac{s_{k-1}^Ty_{k-1}}{y_{k-1}^Ty_{k-1}},
%  \end{aligned}
%\end{equation}
%where $s_{k-1}=x_k-x_{k-1},y_{k-1}=g_k-g_{k-1}$. 
%This choice of $\alpha_k$ can in practice  
%increase the convergence rate if the objective $r(\cdot)$ have more 
%favorable properties~\cite{raydan_1993}.
%Alternatively, $\alpha_k$ can be viewed as 
%a measure of the inverse of a trust-region radius. The larger $\alpha_k$ is, the smaller the step size will be. Hence, 
%$\alpha_k$ can be updated based on how accurate the previous approximation is, as
%in trust-region methods~\cite{Nocedal_book}. This view is adopted in the proposed algorithm. 
%A simple multiplication rule where $\alpha_{k+1}=\eta_{\alpha}\alpha_k,\eta_{\alpha}>1$ could be effective when $\alpha_k$ is 
%increased.
%In all cases, problem specific $\alpha_{max}$ and $\alpha_{min}$ can be assigned to 
%make the algorithm more efficient and robust.
%This is the area of the algorithm that is rich 
%for experimentation.

%It is also possible to gauge $\alpha_k$ better based on function value. 
%If the function value range of $r(\cdot)$ is known, 
%such rules can help convergence.
%For example, one possible way is to  
%require the minimum value of $\phi_k(\cdot)$ to be larger than certain ratio of 
%the function value at $x_k$, as  
%\begin{equation} \label{eqn:rc-quad-appx-2}
% \centering
%  \begin{aligned}
%	  \min_{x \in X}\phi_k(x) \geq \eta_k r_k
%  \end{aligned}
%\end{equation}
%where $\eta_k$ is a chosen coefficient.
%%The parameter $\eta_k$ controls how big 
%%a step $x_{k+1}$ should be from $x_k$ through encouraging or suppressing step size. 
%Using $\eta_k$ as an intermediate parameter, instead of controlling $\alpha_k$ directly, the fixed increase ratio $\eta_{\alpha}$ could be
%applied to $\eta_k$ through trust-region type of control, 
%where $\eta_k$ is decreased if $\rho_k$ is large enough.
%The choice of $\alpha_k$ in this case also depends on local functional quantities such as $g_k$ and $f_k$. 
%
%%The stopping criterion adopted in the algorithm of this work is based on the predicted decrease $\delta_k$ of 
%%the function value. It is effective and often converges fast in practice.
%%Alternatively, 
%%gradient-based stopping criteria such as $\left\lVert g_{k+1}-g_k-\alpha_k(x_{k+1}-x_k) \right\rVert\leq e$,
%%where $e$ is the error tolerance could also be applied. 
%%The left side of the inequality represents the difference between the gradient  
%%of the objective of the master subproblem at $x_{k+1}$ and its approximation at the $k$th step. 
%%Therefore, upon meeting the criteria, the optimality conditions of the $k$th master subproblem
%%with the approximation $\Phi_k(x_{k+1})$ as in~\eqref{eqn:opt-ms-simp-bundle} leads to the master subproblem in~\eqref{eqn:opt-ms-simp} satisfying 
%%the optimality conditions to the degree of $e$ at $x_{k+1}$.


%%The local approximation of the recourse solution is plugged into the algorithm based on sequential quadratic 
%%programming. Algorithm~\ref{} gives the framework of the approach. Conventional sequential quadratic programming
%%constructs a merit function to determine whether a trial step should be taken. In line search methods, the merit
%%function controls the size of the step~\cite{} and includes both the objective and constraint measures.
%%For example, the $l_1$ merit function for an objective function $f(x)$ and constraints $c(x)-s=0$ could be 
%%$\phi_1(x,\mu)=f(x)+\xi||c(x)||_1$, where $\xi$ is the penalty parameter and $||\ ||_1$ is the norm.
%%A step would be accepted if the sufficient decrease condition for line search is satisfied, as
%%$\phi_1(x_k+\beta_kp_k;\xi_k)\leq\phi_1(x_k,\xi_k)+\eta\beta_kD(\phi_1(x_k;\xi);p_k)$, where 
%%$D(\phi_1(x_k;\xi);p_k)$ denotes the directional derivative of $\phi_1$ in the direction $p_k$ and
%%$\eta\in(0,0.5)$. 
%%The line search for $\beta_k$ therefore involves evaluating both the base case and recourse functions
%%multiple times per iteration, which in the case of SCACOPF can be prohibitively expensive. In practice,
%%line search is done using the approximation function for the recourse solution and therefore $f(x)$ 
%%as well\cite{}.
%In practice, $\alpha_k$ can be reduced when $\rho_k$ 
%behaves well, \textit{e.g.}, is close to $1$. In our experience, convergence can be achieved faster 
%while the algorithm remains robust.
%To further speed up convergence, scalar $\alpha_k$ can also be replaced by a diagonal matrix. 
%One way of varying the diagonal values is to take into account the distance 
%between a component of $x$ and its upper and lower bounds. In our numerical 
%experiments, multiple components of the optimization variable $x$ reach their upper/lower bounds.
%Since they are more likely to stay at the bounds, it is reasonable to assign them larger corresponding diagonal values
%of the matrix $\alpha_k$ to encourage movement of other components of $x$. 
%For a first-order algorithm, this could make a difference in
%convergence and proves to be so in our application of SCACOPF problems.

%The Lagrange multiplier is the sensitivity of the constraint violation.
\subsection{Consistency restoration of linearized constraint}\label{sec:lincons}
As mentioned previously, the linearized constraints of the subproblem~\eqref{eqn:opt-ms-simp-bundle} can become infeasible even when the original problem~\eqref{eqn:opt-ms-simp} is feasible, a phenomenon known as inconsistency. To address this possibility, this section introduces and analyzes a consistency restoration algorithm. Whenever the subproblem~\eqref{eqn:opt-ms-simp-bundle} has inconsistent linearized constraints, a penalized subproblem (see~\eqref{eqn:opt-ms-simp-bundle-penal} below) that incorporates a measure of constraints' violation in the objective is solved. The salient idea is to generate a new serious point with \textit{consistent} linearized constraints. 
%It is well known for SQP methods that the linearized constraints could 
%cause inconsistency in solving the subproblems~\cite{Nocedal_book}.
%This means subproblem~\eqref{eqn:opt-ms-simp-bundle} could become infeasible due to the linearized constraints,
%while the original problem~\eqref{eqn:opt-ms-simp} remains feasible. To overcome this, we borrow %an idea
%from sequential linear-quadratic programming (SLQP)~\cite{Nocedal_book,byrd2005} so that whenever 
%inconsistency occurs, the problem
%is addressed in two phases.
The penalized problem might lead to infeasible accumulation points, which is common with penalty methods. 
However, we can minimize the linearized constraint violation for such infeasible points through the update rule of the penalty parameter.
To that end, the algorithm uses an update rule based on a sequential linear-quadratic programming (SLQP) approach~\cite{byrd2005} and it requires solving a so-called feasibility problem in the form of~\eqref{eqn:opt-ms-simp-bundle-fea} below.
%
%The penalty parameter needs to be controlled 
%It is common with penalty methods that the algorithm might generate infeasible accumulation points~\cite{17,Nocedal_book} 
%contingent on the penalty parameter. 
%For the update rule of the penalty parameter,
%we use a sequential linear-quadratic programming (SLQP) approach pioneered by~\cite{byrd2005} that
%relies on solving a feasibility problem.
%The combination of the feasibility and penalty subproblems are called the consistency restoration algorithm.
%
%
%Whenever problem~\eqref{eqn:opt-ms-simp-bundle} has inconsistent linearized constraints,
We first formulate the following penalty problem 
\begin{equation} \label{eqn:opt-ms-simp-bundle-penal-nonsmooth}
 \centering
  \begin{aligned}
   &\underset{\substack{d}}{\text{min}} 
	  & & \pi_k \Phi_k(d) + \norm{c(x_k)+\nabla c(x_k)^T d}_1 & \text{s.t.}
	  & & d_l^k\leq d\leq d_u^k,
  \end{aligned}
\end{equation}
where $\pi_k\geq 0$ is the penalty parameter. 
 To avoid difficulties with the nonsmooth 1-norm, the algorithm solves the following equivalent quadratic programming problem:
\begin{equation} \label{eqn:opt-ms-simp-bundle-penal}
 \centering
  \begin{aligned}
   &\underset{\substack{d,v,w}}{\text{min}} 
	  & & \pi_k \Phi_k(d) + \sum_{j=1}^m (v_j + w_j)  \\
   &\text{s.t.}
	  & & c_j(x_k)+\nabla c_j(x_k)^T d = v_j - w_j, \ j=1,...m,\\
	  &&& d_l^k\leq d\leq d_u^k,\\
	  &&& 0 \leq v, w ,
  \end{aligned}
\end{equation}
where $v,w\in \Rbb^m$ are slack variables. Let $d_k$, $v^k$, and $w^k$ denote the solutions to~\eqref{eqn:opt-ms-simp-bundle-penal}.
The first-order optimality conditions of problem~\eqref{eqn:opt-ms-simp-bundle-penal} for $d$ are
\begin{equation} \label{eqn:simp-bundle-penal-KKT-1}
  \centering
   \begin{aligned}
	   \pi_k \left[g_k + \alpha_k d_k\right] + \sum_{i=1}^m \lambda^{k+1}_j \nabla c_j(x_k)-\zeta_l^{k+1}+\zeta_u^{k+1} =0&,\\
	   \lambda^{k+1}_j \left[c_j(x_k)+\nabla c_j(x_k)^T d_k - v^k_j + w^k_j \right] =0, \ j=1,...m,\\
	   c_j(x_k)+\nabla c_j(x_k)^T d_k - v^k_j + w^k_j =0, \ j=1,...m,\\
	   Z_u^{k+1}(d_k-d_u^k) = 0, Z_l^{k+1}(d_k-d_l^k) = 0&,\\
	   \zeta_u^{k+1},\zeta_l^{k+1},d_k+x_k,x_u-x_k-d_k\geq 0&.\\
   \end{aligned}
 \end{equation}
Here, $\lambda^{k+1}\in\Rbb^m$, $\zeta_u^{k+1}\in \Rbb^n$, and $\zeta_l^{k+1}\in \Rbb^n$ are the Lagrange multipliers for the constraints, while $Z_u^{k+1}$ and $Z_l^{k+1}$ are diagonal matrices with values $\zeta_u^{k+1}$ and $\zeta_l^{k+1}$, respectively.
The remaining optimality conditions on slack variables $v$ and $w$ are 
\begin{equation} \label{eqn:simp-bundle-penal-KKT-2}
  \centering
   \begin{aligned}
	   1-\lambda^{k+1}_j - p^{k+1}_j =0, \ j=1,...m,\\
           1+\lambda^{k+1}_j-q^{k+1}_j=0, \ j=1,...m,\\
	   P^{k+1} v^k  = 0, Q^{k+1} w^k = 0&,\\
	   v^k,w^k,p^{k+1},q^{k+1} \geq 0&,\\
   \end{aligned}
 \end{equation}
where $p^{k+1}\in\Rbb^m$ and $q^{k+1}\in\Rbb^m$ are the Lagrange multipliers for bound constraints on $v^k$ and $w^k$, respectively, and $P^{k+1}$ and $Q^{k+1}$ are diagonal matrices whose diagonal entries are elements of $p^{k+1}$ and $q^{k+1}$, respectively. 
Based on whether the slack variable bound constraints are active, the relations among the multipliers 
can be simplified. 
To proceed, we define the sign function $\sigma_j^k:\Rbb^n\to\Rbb$, $j=1,\dots,m$ of $d$ by
\begin{equation} \label{eqn:opt-ms-simp-sign}
 \centering
  \begin{aligned}
	  \sigma_j^k(d)  =  
	  \begin{cases}
		  -1,  
		       & c_j(x_k)+\nabla c_j(x_k)^T d < 0, \\  
		  \phantom{-}0,
		  & c_j(x_k) + \nabla c_j(x_k)^T d = 0,\\
		  \phantom{-}1,
		  & c_j(x_k) + \nabla c_j(x_k)^T d > 0.
    \end{cases}
  \end{aligned}
\end{equation}
In addition, for $d_k$, we define
%we divide the constraints into two sets based on the value of $ c_j(x_k)+ \nabla c_j(x_k)^T d_{k}$. 
%For simplicity, the two sets are referred to as the set of active and inactive equality constraints as we do without slack variables. 
the active equality constraint set as
\begin{equation} \label{eqn:opt-ms-simp-bundle-fea-A}
   \centering
    \begin{aligned}
     A_k = \{ 1\leq j\leq m|c_j(x_k)+\nabla c_j(x_k)^T d_{k} = 0\},
     \end{aligned}
\end{equation}
and the inactive equality constraint set as
\begin{equation} \label{eqn:opt-ms-simp-bundle-fea-I}
  \centering
    \begin{aligned}
      V_k = \{ 1\leq j\leq m|c_j(x_k)+\nabla c_j(x_k)^T d_{k} \neq 0\}.
    \end{aligned}
\end{equation}
  The optimality conditions~\eqref{eqn:simp-bundle-penal-KKT-2} are integrated into~\eqref{eqn:simp-bundle-penal-KKT-1}
in the following lemma.

\begin{lemma}\label{lem:lambda-relaxed-prop}
	For all $j\in V_k$, $\lambda_j^{k+1} = \sigma_j^k(d_k)$. Also, for all $j\in A_k$, 
        $\lambda_j^{k+1}\in [-1,1]$.
\end{lemma}
\begin{proof}
	Note first that for any $ j\in[1,m]$, the slack variable solutions satisfy $v^k_j w^k_j = 0$. 
	%In other words, 
	%due to the bound constraints on $v,w$  and their presence in the objective, at least one of their $j$th
        %component is $0$.
	We consider the three cases given by the value of %$c_j(x_k)+\nabla c_j(x_k)^T d_k$, which corresponds 
	%to the three values of 
	$\sigma_j^k(d_k),j=1,\dots,m$.
	%The first two cases both have $j\in V_k$.
	If $\sigma_j^k(d_k)=1$, by the third equation in~\eqref{eqn:simp-bundle-penal-KKT-1}, $v_j^k>0$ and $w_j^k=0$.
	From~\eqref{eqn:simp-bundle-penal-KKT-2}, 
        $p^{k+1}_j=0$. Then, by the first equation in~\eqref{eqn:simp-bundle-penal-KKT-2}, $\lambda_j^{k+1}=1$.
	Similarly, if $\sigma_j^k(d_k)=-1$, 
        one obtains $q^{k+1}_j=0$ and $\lambda_j^{k+1}=-1$. The first part of the Lemma is proven.

	In the last case, $j\in A_k$, \textit{i.e.}, $\sigma_j^k(d_k)=0$. By the third equation in~\eqref{eqn:simp-bundle-penal-KKT-1}, we have $v_j^k=0$ and $w_j^k=0$.  
We sum and subtract the first two equations in~\eqref{eqn:simp-bundle-penal-KKT-2} to obtain 
%      \begin{equation} \label{eqn:lambda-pq}
%       \centering
%        \begin{aligned}
		$\lambda_j^{k+1} = \frac{1}{2}(q_j^{k+1}-p_j^{k+1})$ and %\\
		$p_j^{k+1}+q_j^{k+1}=2$. %\\
        %\end{aligned}
       %\end{equation}
	The bound constraints on $p^{k+1}$ and $q^{k+1}$ and the latter equation implies $0\leq p_j^{k+1}$ and $q_j^{k+1}\leq 2$; finally,
	the former equation implies $\lambda_j^{k+1}\in [-1,1]$.
\end{proof}

Similar to~\eqref{def:pd}, we define $\delta_k^{\pi_k}$ to be the predicted change in objective of the penalty subproblem~\eqref{eqn:opt-ms-simp-bundle-penal} with penalty $\pi_k$, which based on~\eqref{eqn:opt-ms-simp-bundle-penal-nonsmooth} is 
\begin{equation}\label{def:pd-penal}
   \begin{aligned}
	   \delta_k^{\pi_k} =& \pi_k\left(-g_k^T d_k -\frac{1}{2}\alpha_k \norm{d_k}^2\right) +\norm{c(x_k)}_1 -\norm{c(x_k)+\nabla c(x_k)^T d_k}_1.\\
	  % =&\pi_k \delta_k - \sum_{j\in V_k}\sigma_j \nabla c_j(x_k)^T d_k.
   \end{aligned}
\end{equation}
The ratios $\rho_k$~\eqref{eqn:decrease-ratio-1} and $\rho_k^{\beta}$~\eqref{eqn:decrease-ratio-beta} are again used to address the nonsmoothness of $r$. 
The algorithm also requires line search on the constraints to obtain a serious step 
$x_{k+1}=x_k+\beta_k d_k$, $\beta_k\in (0,1]$. 
To simplify the analysis, we adopt in this section $\eta_{\gamma}^-=\eta_{\gamma}^+=1$ and $\eta_l^-=\eta_l^+=1$, 
making the definition of $\rho_k,\rho_k^{\beta}$ in~\eqref{eqn:decrease-ratio-1} and~\eqref{eqn:decrease-ratio-beta} identical 
across branches.
Thus, regardless of the value of $\alpha_k$, 
a serious step $x_{k+1}$ satisfies 
$r(x_k)-r(x_{k+1}) > \Phi_k(0)-\Phi_k(\beta_kd_k)$ and $r(x_k)-r(x_{k}+d_k) > \Phi_k(0)-\Phi_k(d_k)$. 

The merit function and line search conditions for consistency restoration are 
\begin{equation}\label{def:merit-fea}
   \begin{aligned}
	   \phi_{1\pi_k}(x)  =  r(x) + \frac{1}{\pi_k} \norm{c(x)}_1,
   \end{aligned}
\end{equation}
and 
\begin{equation}\label{eqn:line-search-cond-penal}
   \begin{aligned}
   \centering
	   \frac{1}{\pi_k} \norm{c(x_k)}_1  +  \frac{\beta_k}{\pi_k} (\lambda^{k+1})^T \nabla c(x_k)^T d_k  \geq
	   \frac{1}{\pi_k} \norm{c(x_{k+1})}_1 -\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2. 
   \end{aligned}
\end{equation}

To update the penalty parameter, 
the following feasibility problem is also solved:
\begin{equation} \label{eqn:opt-ms-simp-bundle-fea}
 \centering
  \begin{aligned}
   &\underset{\substack{d}}{\text{min}} 
	  & & \norm{c(x_k) + \nabla c(x_k)^T d}_1 &\text{s.t.} & & d_l^k\leq d\leq d_u^k.
  \end{aligned}
\end{equation}
%where the bound constraints, which are already linear, are enforced. 
%While~\eqref{eqn:opt-ms-simp-bundle-fea} appears to have nonsmooth objective, it can be transformed to a smooth one using slack variables~\cite{Nocedal_book}.
%We know from intermediate value 
%theorem for connected sets, given that consistent linearized constraints form a convex feasible set, 
%$c_j(x_k) + \nabla c_j(x_k)^T d, j\in V_k$ is either positive or negative for all $x$ satisfying
%the remaining constraints. \ccom{[[the previous sentence is a mess, not clear clear at all that you actually want the signs to not change in a neighborhood; also not clear how you argue this is the case... what is the convex feasible set? what is the connect set? what are the remaining constraints; please rewrite it]]}
%Let us define by $\sigma_j$ the sign of the $j$th violated constraint, that is $\sigma_j=1$ if $c_j(x_k)$ is positive and $\sigma_j=-1$ if $c_j(x_k)$ is negative, for all $j\in V_k$. We introduced a penalty subproblem  in the form of 
%\begin{equation} \label{eqn:opt-ms-simp-bundle-penal}
% \centering
%  \begin{aligned}
%   &\underset{\substack{x\in \Rbb^n}}{\text{min}} 
%	  & & \pi_k \Phi_k(d) +  \sum_{j\in V_k} \sigma_j [\nabla c_j(x_k)^T d] \\
%   &\text{s.t.}
%	  & & c_j(x_k) + \nabla c_j(x_k)^T d =0, \ j\in A_k\\ 
%	  &&& d_l\leq d\leq d_u,
%  \end{aligned}
%\end{equation}
%where $\pi_k$ is the penalty parameter. 
%We remark that $\sigma_j [\nabla c_j(x_k)^T d], j\in V_k$ is affine, hence the objective remains upper-$C^2$. As a consequence, the algorithm we propose for consistency restoration in this section builds on Algorithm 1.
%As in many penalty methods, we distinguish the case where $\pi_k$ is bounded above $0$ and where 
%it converges to $0$. \ccom{[[I am not sure this is a good place to mention this]]} We call $\pi_k$ stabilized if it stops changing for $k$ large enough. \ccom{[[not sure this is relevant at this point]]}
Denote by $d_{k}^f$ the solution to~\eqref{eqn:opt-ms-simp-bundle-fea} and by $\delta_k^f$ its predicted decrease,
whose form is 
\begin{equation}\label{def:pd-fea} 
   \begin{aligned}
	   \delta_k^f = \norm{c(x_k)}_1-\norm{c(x_k)+\nabla c(x_k)^T d_k^f}_1.
   \end{aligned}
\end{equation}
Notice that $\delta_k^f\geq 0$. This value is compared against $\delta_k^{\pi_k}$. 
%The optimality conditions for~\eqref{eqn:opt-ms-simp-bundle-penal} are
%	\begin{equation} \label{eqn:simp-bundle-penal-KKT}
%  \centering
%   \begin{aligned}
%	   \pi_k \left[g_k + \alpha_k d_k\right] + \sum_{j\in V_k}\sigma_j \nabla c_j(x_k) 
%	   +\sum_{j\in A_k}\lambda_j^{k+1} \nabla c_j(x_k)   -\zeta_l^{k+1}+\zeta_u^{k+1} =0&,\\
%	   Z_u^{k+1}(d_k-d_u) = 0, Z_l^{k+1}(d_k-d_l) = 0&,\\
%	   \lambda_j^{k+1} \left[c_j(x_k)+\nabla c_j(x_k)^Td_k\right] = 0,\ j\in A_k&,\\
%	   \zeta_u^{k+1},\zeta_l^{k+1},d_k+x_k,x_u-x_k-d_k\geq 0&,\\
%	   c_j(x_k)+\nabla c_j(x_k)^Td_k= 0,\ j\in A_k&.
%   \end{aligned}
% \end{equation}
%where $\lambda^{k+1}\in \Rbb^{|A_k|}$ is a vector of Lagrange multipliers for linearized constraints and $\zeta_u^{k+1}$ and $\zeta_l^{k+1}\in \Rbb^n$ are the Lagrange multipliers for the bound constraints. 

The consistency restoration algorithm is given in Algorithm~\ref{alg:simp-bundle-const}. It activates in 
Algorithm~\ref{alg:simp-bundle} when inconsistency occurs at step 3 and exits after one serious step iteration in step 12 of Algorithm~\ref{alg:simp-bundle-const}. However, 
it is possible that the linearized constraints remain inconsistent and   
Algorithm~\ref{alg:simp-bundle-const} is called repeatedly. 
In this case, the update rule of the penalty parameter ensures that the algorithm converges toward critical points for linearized constraint violations. A point $\bar{x}$ is called a critical point of the linearized constraint violation of $c$ if $\delta_k^f=0$ at $\bar{x}$. Such a critical point can be either feasible or infeasible to the original problem~\eqref{eqn:opt-ms-simp}. 
%This is further elaborated and analyzed later in this section. 
\begin{algorithm}
% \DontPrintSemicolon
% \SetAlgoNoLine 
   \caption{Simplified bundle method: consistency restoration}\label{alg:simp-bundle-const}
	\begin{algorithmic}[1]
		\STATE{Given $x_k$, $\alpha_k$, $r_k$, $g_k$, $\theta_k$ and $\epsilon$ from Algorithm~\ref{alg:simp-bundle}, choose coefficient $\eta_{\pi}\in (0,1), \eta_f\in (0,1)$ and error tolerance $\epsilon^f\geq 0$.
	If $\pi_{k-1}$ does not exist, let $\pi_k=\frac{1}{\theta_k}$. Otherwise, let $\pi_k=\min{(\pi_{k-1},\frac{1}{\theta_k})}$. 
	    Solve~\eqref{eqn:opt-ms-simp-bundle-penal} with $\pi_k$ and obtain $d_k$.}
	%\IF{$\delta_k^{\pi_k} < \epsilon$}
        %  \STATE{Stop the iteration and exit the algorithm.}
        %\ENDIF
	    \STATE{Solve feasibility problem~\eqref{eqn:opt-ms-simp-bundle-fea} to obtain solution $d_k^f$ and compute 
	    $\delta_k^f$ in~\eqref{def:pd-fea}.}
	\IF{$\delta_k^f < \epsilon^f$}
          \STATE{Stop the iteration and exit the algorithm.}
        \ENDIF
	\WHILE{$\delta_k^{\pi_k}<\eta_f \delta_k^f$}
	  \STATE{Reduce $\pi_k$ through $\pi_k = \eta_{\pi} \pi_{k}$ and re-solve~\eqref{eqn:opt-ms-simp-bundle-penal} with the updated $\pi_k$.}
	\ENDWHILE
	\STATE{Obtain the solution $d_k$. %and Lagrange multipliers $\lambda^{k+1}$ given $\pi_k$.
	    Evaluate $r(x_k+d_k)$, $\delta_k$ in~\eqref{def:pd} and $\rho_k$ in~\eqref{eqn:decrease-ratio-1}.}
	\IF{$\rho_k > 0$}
	  \STATE{Find the line-search parameter $\beta_k>0$ using backtracking, starting at $\beta_k=1$ and halving 
		  if too large, such that~\eqref{eqn:line-search-cond-penal} is satisfied. Compute $\rho_k^{\beta}$ in~\eqref{eqn:decrease-ratio-beta}.}
            \IF{$\rho_k^{\beta} < 0$}
	     \STATE{Break and go to 16.}
	    \ENDIF
	    \STATE{Take the serious step $x_{k+1} = x_k+\beta_k d_k$.
	    Exit consistency restoration. Go back to Algorithm~\ref{alg:simp-bundle} and start a new iteration.}
       \ELSE
	   \STATE{Reject the trial step and update $\alpha_k$ with $\alpha_{k+1}=\eta_{\alpha}\alpha_k$.
            Go back to step 1.}
       \ENDIF
    \end{algorithmic}
\end{algorithm}

While Algorithm~\ref{alg:simp-bundle-const} solves a penalized subproblem instead, 
it includes all the elements in Algorithm~\ref{alg:simp-bundle} to deal with the nonsmoothness of $r$, including the update rule for $\alpha_k$.
Thus, we can reuse many analyses from Section~\ref{sec:alg-convg}  
and only provide rigorous proofs if necessary.
%Since the acceptance and rejection of a potential step is based on $\rho_k$ and $\rho_k^{\beta}$, which in turn 
%solely relies on properties of $r(\cdot)$, 
First, Lemma~\ref{lem:sufficientdecrease} holds true, as in the form of the following lemma.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Lemma: finite number of rejected steps
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:sufficientdecrease-penal}
	Under the Assumption~\eqref{assp:upperC2}, the consistency restoration Algorithm \ref{alg:simp-bundle-const} produces a finite number 
	of rejected steps. Consequently, the parameter $\alpha_k$ of Algorithm~\ref{alg:simp-bundle-const} stabilizes, \textit{i.e.}, there exists $k$ such that $\alpha_t = \alpha_k$ for all $t\geq k$. 
\end{lemma}
\begin{proof}
	Since Algorithm~\ref{alg:simp-bundle-const} has identical mechanism for rejecting steps and increasing $\alpha_k$ to Algorithm~\ref{alg:simp-bundle}, which only relies on the property of $r$, the proof of Lemma~\ref{lem:sufficientdecrease} can be directly applied here.
%; furthermore, both lemmas only involve the upper-$C^2$ objective $r(\cdot)$.
%Since $c$ is smooth and $r$ is upper-$C^2$, the penalized objective would continue to be upper-$C^2$. 
	Only a finite number of rejected steps are needed to achieve $\alpha_k>2C$, which guarantees $\rho_k>0$, $\rho_k^{\beta}>0$, and produces a serious step. If $\alpha_k\leq 2C$ for all $k$, then only finite number of rejected steps are generated, which also means all steps are serious steps, \textit{i.e.}, $\rho_k>0,\rho_k^{\beta}>0$, for $k$ large enough.
As a result, there exists a $k$ such that $\alpha_t=\alpha_k$ for $t\geq k$  (see proof of Lemma~\ref{lem:sufficientdecrease}), with a finite number of rejected steps produced.
\end{proof}
The following lemma shows that the update rule for $\pi_k$ in Algorithm~\ref{alg:simp-bundle-const} is well-defined.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Lemma: penalty parameter update
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:consistency-penal-defined}
	Steps 5-6 in Algorithm~\ref{alg:simp-bundle-const} terminate successfully, \textit{i.e.}, there exists a $\pi_k>0$ such that $\delta_k^{\pi_k}\geq \eta_f \delta_k^f$ and such a $\pi_k$ can be found in a finite number of steps.  
\end{lemma}
\begin{proof}
	%We need to show that there exists $\pi_k > 0$ such that $\delta_k^{\pi_k} \geq \eta_{\pi}\delta_k^f$. 
	%The decrease in the penalized problem~\eqref{eqn:opt-ms-simp-bundle-penal} is , 
	%where $d_k=x_{k+1}-x_k$ with $x_{k+1}$ the solution to~\eqref{eqn:opt-ms-simp-bundle-penal}. 
	%Denote $d_k^f = x_{k+1}^f-x_k$, where $x_{k+1}^f$ is the solution to~\eqref{eqn:opt-ms-simp-bundle-fea}.
	%The decrease in objective for the feasibility problem is defined as $\delta_k^f = $
	%then $\norm{c(x_k)+\nabla c(x_k)^T d_k}_1 \geq \norm{c(x_k)+\nabla c(x_k)^Td_k^f}_1$.
	%Equivalently, 
	%%$\sum_{j\in V_k}\sigma_j (c_j(x_k)+\nabla c_j(x_k)^T d_k) \geq \sum_{j\in V_k}\sigma_j(c_j(x_k)+\nabla c_j(x_k)^Td_k^f)$ and thus 
	%$\sum_{j\in V_k}\sigma_j \nabla c_j(x_k)^T d_k \geq \sum_{j\in V_k}\sigma_j \nabla c_j(x_k)^Td_k^f$.
	Since $d_k$ is the solution to~\eqref{eqn:opt-ms-simp-bundle-penal} and~\eqref{eqn:opt-ms-simp-bundle-penal-nonsmooth}, by~\eqref{def:pd-penal} we can write 
   \begin{equation} \label{eqn:simp-bundle-fea-finite}
   \centering
    \begin{aligned}
	    \delta_k^{\pi_k} \geq& \pi_k\left(-g_k^T d_k^f  - \frac{1}{2} \alpha_k \norm{d_k^f}^2\right) 
	    +\norm{c(x_k)}_1 - \norm{c(x_k)+ \nabla c(x_k)^T d_k^f}_1. \\
    \end{aligned}
   \end{equation}
   By~\eqref{def:pd-fea} and Cauchy-Schwarz inequality,
   \begin{equation} \label{eqn:simp-bundle-fea-finite-2}
   \centering
    \begin{aligned}
	    \delta_k^{\pi_k} \geq& 
		     \pi_k\left(-g_k^T d_k^f  - \frac{1}{2} \alpha_k \norm{d_k^f}^2\right) + \delta_k^f \geq \pi_k\left(-\norm{g_k}\norm{d_k^f} - \frac{1}{2}\alpha_k\norm{d_k^f}^2\right)+ \delta_k^f.\\
    \end{aligned}
   \end{equation}
	From Lemma~\ref{lem:sufficientdecrease-penal} and Lipschitz continuity of $r$, $d_k^f$, $g_k$, and $\alpha_k$ are all bounded. Assigning $D = \norm{d_u^k-d_l^k}=\norm{x_u}$, we derive the condition on $\pi_k$ to ensure $\delta_k^{\pi_k}\geq \eta_f \delta_k^f$: 
   \begin{equation} \label{eqn:simp-bundle-fea-pi}
   \centering
    \begin{aligned}
	    \pi_k  \leq  \frac{(1-\eta_f)\delta_k^f}{ \norm{g_k} D + \frac{1}{2}\alpha_k D^2 }.\\
    \end{aligned}
   \end{equation}
	Thus, such $\pi_k>0$ exists as long as $\delta_k^f>0$. And since $\pi_k$ is reduced through $\eta_{\pi}<1$, only a finite number of steps are needed to obtain such a $\pi_k$ in step 8.
	If $\delta_k^f = 0$ and consistency restoration Algorithm~\ref{alg:simp-bundle-const} is still called, it would terminate at step 4. 
\end{proof}


\begin{lemma}\label{lem:line-search-merit-2}
	Given $\pi_k>0$ and Assumption~\eqref{assp:boundedHc}, the line search step 9 of Algorithm~\ref{alg:simp-bundle-const} finds $\beta_k\in (0,1]$ satisfying the line search condition~\eqref{eqn:line-search-cond-penal} in a finite number of steps.
\end{lemma}
\begin{proof}
	Since constraints $c$ are smooth, by Taylor expansion of its $jth$ component, $1\leq j \leq m$, for $x_{k+1}=x_k+\beta_k d_k$
   %\begin{equation} \label{eqn:simp-bundle-fea-c-taylor}
   %\centering
   % \begin{aligned}
%	    c_j(x_k+d_k) - c_j(x_k)  = \nabla c_j(x_k)^T d_k  + \frac{1}{2} d_k^T H_{k}^j d_k,\\
 %   \end{aligned}
 %  \end{equation}
       \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-1}
         \centering
         \begin{aligned}
		 c_j(x_{k+1})  = & c_j(x_k)+ \beta_k \nabla c_j(x_k)^T d_{k} + \frac{1}{2}\beta_k^2 d_k^T H_{k\beta}^{j} d_k,\\
      \end{aligned}
     \end{equation}
	where $H_{k\beta}^j$ depends on both $x_k$ and $d_k$. 
	By Assumption~\ref{assp:boundedHc} and triangle inequality, we have
   \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2}
   \centering
    \begin{aligned}
	    |c_j(x_{k+1})|  &= | c_j(x_k)+ \beta_k \nabla c_j(x_k)^T d_{k}+ \frac{1}{2}\beta_k^2 d_k^T H_{k\beta}^{j} d_k|\\
	    &\leq | c_j(x_k) + \beta_k \nabla c_j(x_k)^T d_{k}| + \beta_k^2 H^{c}_u \norm{d_k}^2\\
	     &= \left|(1-\beta_k) c_j(x_k) + \beta_k \left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right]\right|+\beta_k^2 H^{c}_u \norm{d_k}^2\\ 
	      & \leq (1-\beta_k)| c_j(x_k)| + \beta_k |c_j(x_k)+ \nabla c_j(x_k)^T d_{k}|+ \beta_k^2 H^{c}_u \norm{d_k}^2 . 
    \end{aligned}
   \end{equation}
	Applying the definition~\eqref{eqn:opt-ms-simp-sign} of $\sigma_j^k$ to~\eqref{eqn:simp-bundle-fea-c-ls-pf-2}, we can write 
   %\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.1}
   %\centering
   % \begin{aligned}
%	    |c_j(x_k)+ \nabla c_j(x_k)^T d_{k}| = \sigma_j^k(d_k) \left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right].
%    \end{aligned}
%   \end{equation}
	%Since the function $d\mapsto|c_j(x_k)+\nabla c_j(x_k)^T d|$ is convex in $d$,
	%by taking its value at $d=0,d=d_k$ and $\beta_k d_k$, we have by convexity 
 %\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.2}
 %  \centering
 %   \begin{aligned}
%	    | c_j(x_k) + \beta_k \nabla c_j(x_k)^T d_{k}|  & \leq |(1-\beta_k) c_j(x_k) + \beta_k \left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right]|\\ 
%	      & \leq (1-\beta_k)| c_j(x_k)| + \beta_k |c_j(x_k)+ \nabla c_j(x_k)^T d_{k}|. 
 %   \end{aligned}
 %  \end{equation}
	%Applying~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.1} to~\eqref{eqn:simp-bundle-fea-c-ls-pf-2} gives us 
\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.3}
   \centering
    \begin{aligned}
	    |c_j(x_{k+1})|  %& \leq (1-\beta_k)| c_j(x_k)| + \beta_k |c_j(x_k)+ \nabla c_j(x_k)^T d_{k}| + \beta_k^2 H^{c}_u \norm{d_k}^2\\
		  & \leq (1-\beta_k)|c_j(x_k)| + \beta_k \sigma_j^k(d_k)\left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right] + \beta_k^2 H^{c}_u \norm{d_k}^2.
    \end{aligned}
   \end{equation}
	Let us denote the cardinality of $A_k$ and $V_k$ by $|A_k|$ and $|V_k|$, respectively. By summing up~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.3} over $j\in V_k$ and noting that $|c_j(x_k)|\geq \sigma_j^k(d_k) c_j(x_k)$, we have
   \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.5}
     \centering
      \begin{aligned}
	      \sum_{j\in V_k}|c_j(x_{k+1})|  \leq& 
	       \sum_{j \in V_k}  |c_j(x_k)|+\beta_k\sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^Td_k 
	      + |V_k|\beta_k^2 H^{c}_u \norm{d_k}^2.\\
      \end{aligned}
    \end{equation}
	Similarly, we sum up~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.3} over $j\in A_k$ and use the definition in~\eqref{eqn:opt-ms-simp-bundle-fea-A} to write 
   \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.6}
     \centering
      \begin{aligned}
\sum_{j\in A_k}|c_j(x_{k+1})|  \leq& 
	      (1-\beta_k)\sum_{j \in A_k}  |c_j(x_k)| + |A_k| \beta_k^2 H^{c}_u \norm{d_k}^2. \\
      \end{aligned}
    \end{equation}
	%Further, by~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.5} and~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.6}, we have 
%\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-2.8}
%     \centering
%      \begin{aligned}
%	      \sum_{j\in V_k}\left(|c_j(x_k)|-|c_j(x_{k+1})|\right)  \geq& 
%	       -\beta_k \sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^Td_k 
%	      - |V_k|\beta_k^2 H^{c}_u \norm{d_k}^2,\\
%	      \sum_{j\in A_k}\left(|c_j(x_k)|-|c_j(x_{k+1})|\right)  \geq& 
%	    \beta_k  \sum_{j \in A_k}  |c_j(x_k)| - |A_k| \beta_k^2 H^{c}_u \norm{d_k}^2. \\
%      \end{aligned}
%    \end{equation}
    Summing the two equations in~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.5} and~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.6}
    %~\eqref{eqn:simp-bundle-fea-c-ls-pf-2.8} 
    and using $|A_k|+|V_k|=m$ gives us 
\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-3}
     \centering
      \begin{aligned}
	      \norm{c(x_k)}_1-\norm{c(x_{k+1})}_1 \geq  
	    \beta_k  \sum_{j \in A_k}  |c_j(x_k)|   -\beta_k \sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^T d_k 
	     - m\beta_k^2 H^{c}_u \norm{d_k}^2. \\
      \end{aligned}
    \end{equation}
    From Lemma~\ref{lem:lambda-relaxed-prop} and the definition~\eqref{eqn:opt-ms-simp-bundle-fea-A} of $A_k$, we can write
\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-3.1}
     \centering
      \begin{aligned}
	      \sum_{j=1}^m \lambda_j^{k+1}\nabla c_j(x_k)^T d_k =& \sum_{j\in V_k} \lambda_j^{k+1} \nabla c_j(x_k)^T d_k +\sum_{j\in A_k} \lambda_j^{k+1} \nabla c_j(x_k)^T d_k\\
	      =& \sum_{j\in V_k} \sigma_j^k(d_k) \nabla c_j(x_k)^T d_k -\sum_{j\in A_k} \lambda^{k+1}_j  c_j(x_k).\\
	      \geq& \sum_{j\in V_k} \sigma_j^k(d_k) \nabla c_j(x_k)^T d_k -\sum_{j\in A_k}  |c_j(x_k)|.\\
      \end{aligned}
    \end{equation}
    The inequality in~\eqref{eqn:simp-bundle-fea-c-ls-pf-3.1} comes from the second part of Lemma~\ref{lem:lambda-relaxed-prop}, 
    namely $\lambda^{k+1}_j\in [-1,1]$.
	Through basic algebraic calculations and applying~\eqref{eqn:simp-bundle-fea-c-ls-pf-3} and~\eqref{eqn:simp-bundle-fea-c-ls-pf-3.1} 
   \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-3.5}
   \centering
    \begin{aligned}
	    & \frac{1}{\pi_k} \norm{c(x_k)}_1 -\frac{1}{\pi_k}\norm{c(x_{k+1})}_1 + \frac{\beta_k}{\pi_k} \sum_{j=1}^m \lambda^{k+1}_j\nabla c_j(x_k)^T d_k
	     \geq \\
	    &\qquad \frac{\beta_k}{\pi_k} \sum_{j \in A_k}  |c_j(x_k)|  
	      -\frac{\beta_k}{\pi_k} \sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^T d_k
	      - \frac{1}{\pi_k} m\beta_k^2 H^{c}_u \norm{d_k}^2 \\ 
	    & \qquad+ \frac{\beta_k}{\pi_k}\sum_{j\in V_k} \sigma_j^k(d_k) \nabla c_j(x_k)^T d_k
	     - \frac{\beta_k}{\pi_k} \sum_{j\in A_k} | c_j(x_k) | \geq 
	    - \frac{1}{\pi_k} m \beta_k^2 H^{c}_u \norm{d_k}^2.
    \end{aligned}
   \end{equation}
   Thus, if $\beta_k$ satisfies 
   %\begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-4}
   %\centering
   % \begin{aligned}
	    $0< \beta_k \leq \frac{\eta_{\beta} \alpha_k \pi_k}{2m H^c_u }$,
    %\end{aligned}
   %\end{equation}
   where both the denominator and numerator are positive and independent of line search, the line search condition~\eqref{eqn:line-search-cond-penal} is
   satisfied.
Using ceiling function $\lceil\cdot \rceil$, we have 
   \begin{equation} \label{eqn:simp-bundle-fea-c-ls-pf-5}
   \centering
    \begin{aligned}
	    \beta_k \geq \frac{1}{2} ^{\lceil \log_{\frac{1}{2}} \frac{\eta_{\beta} \alpha_k\pi_k}{2 m H^c_u} \rceil}.
    \end{aligned}
   \end{equation}
	For each $k$, as ${\pi_k} >0$, the line search successfully exits after a finite number of steps. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent We do point out that if $\pi_k\to 0$, $\beta_k\to 0$ as well.
One can prove the decrease in merit function similarly to Lemma~\ref{lem:sufficientdecrease-merit}. 
\begin{lemma}\label{lem:sufficientdecrease-merit-penal}
	The serious step $x_{k+1}=x_k+\beta_k d_k$ is a descent step for the merit function~\eqref{def:merit-fea} if 
	$\beta_k$ is obtained through step 9 in Algorithm~\ref{alg:simp-bundle-const}. Further, if $\pi_k$ stabilizes above $0$,
	\textit{i.e.}, there exists $k$ such that $\pi_t=\pi_k>0$ for all $t\geq k$, the reduction of the merit function 
	satisfies $\phi_{1\pi_k}(x_k)-\phi_{1\pi_k}(x_{k+1})>c_{\phi}^{\pi}\norm{d_k}^2$ for some $c_{\phi}^{\pi}>0$.
\end{lemma}
\begin{proof}
	Since  $\rho_k>0,\rho_k^{\beta}>0$ at any serious step,  and $\eta_l^+=\eta_l^-=\eta_{\gamma}^+=\eta_{\gamma}^-=1$, we can compactly write based on definitions~\eqref{eqn:decrease-ratio-1},~\eqref{eqn:decrease-ratio-beta} and~\eqref{eqn:opt-ms-appx-rec-merit-beta} that
         %\begin{equation} \label{eqn:opt-ms-appx-rec-obj4}
         %\centering
         %\begin{aligned}
	%	 r_k - r(x_k+d_k) 
%			>   \Phi_k(0) -\Phi_k(d_k) \ \textnormal{ and } \
%		 r_k - r(x_{k+1}) 
%			>   \Phi_k(0) -\Phi_k(\beta_k d_k).
%         \end{aligned}
%       \end{equation}
	%Using the upper-$C^2$ property of $r$, as in 
	%from Lemma~\ref{lem:sufficientdecrease-merit}, we have  
\begin{equation} \label{eqn:simp-bundle-merit-penal-pf-1}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) >& -\beta_k g_{k}^Td_k -\frac{1}{2}\alpha_k\beta_k^2 \norm{d_k}^2. \\
  \end{aligned}
\end{equation}
	Let us rearrange the first equation in the KKT conditions~\eqref{eqn:simp-bundle-penal-KKT-1} to obtain 
\begin{equation} \label{eqn:simp-bundle-penal-merit-pf-1}
  \centering
   \begin{aligned}
	   \pi_k \left[g_k + \alpha_k d_k \right] = -\sum_{j=1}^m\lambda_j^{k+1} \nabla c_j(x_k) 
	     + \zeta_l^{k+1}-\zeta_u^{k+1}.\\
   \end{aligned}
 \end{equation}
	Taking the dot product with $-d_k$ on both sides of~\eqref{eqn:simp-bundle-penal-merit-pf-1} leads to
\begin{equation} \label{eqn:simp-bundle-penal-merit-pf-2}
  \centering
   \begin{aligned}
	   - \pi_k \left[g_k^Td_k + \alpha_k\norm{d_k}^2\right] =& \sum_{j=1}^m\lambda^{k+1}_j \nabla c_j(x_k)^T d_k 
	    -d_k^T \zeta_l^{k+1} + d_k^T \zeta_u^{k+1}.\\
   \end{aligned}
 \end{equation}
	Recall that $d_l^k=-x_k$ and $d_u^k=x_u-x_k$.
	Using the fourth and fifth equations in~\eqref{eqn:simp-bundle-penal-KKT-1}, we have
\begin{equation} \label{eqn:simp-bundle-penal-merit-pf-2.3}
  \centering
   \begin{aligned}
	   -d_k^T \zeta_l^{k+1} + d_k^T \zeta_u^{k+1} =& -(d_k-d_l^k+d_l^k)^T\zeta_l^{k+1}+(d_k-d_u^k+d_u^k)^T\zeta_u^{k+1}\\
					       =& x_k^T \zeta_l^{k+1} +(x_u-x_k)^T \zeta_u^{k+1}
					       \geq 0.
   \end{aligned}
 \end{equation}
	The inequality above is obtained from the bound constraints, namely, $0\leq x_k\leq x_u$, $\zeta_u^{k+1}\geq 0$, and $\zeta_l^{k+1}\geq 0$.
	Applying~\eqref{eqn:simp-bundle-penal-merit-pf-2.3} to~\eqref{eqn:simp-bundle-penal-merit-pf-2}, we have
\begin{equation} \label{eqn:simp-bundle-penal-merit-pf-2.5}
  \centering
   \begin{aligned}
	   -\pi_k  \left[g_k^Td_k + \alpha_k\norm{d_k}^2\right] %=& \sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k)^T d_k 
	   %-(d_k-d_l^k+d_l^k)^T\zeta_l^{k+1}+d_k^T\zeta_u^{k+1}\\
           % =& \sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k)^T d_k 
	   %+x_k^T\zeta_l^{k+1}+(d_k-d_u^k+d_u^k)^T\zeta_u^{k+1}\\
	   %=& \sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k 
	   % +x_k^T \zeta_l^{k+1}
	   %+(x_u-x_k)^T \zeta_u^{k+1}\\
	   \geq& \sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k. 
   \end{aligned}
 \end{equation}
	Since $\beta_k\in (0,1]$, one can multiply by $\frac{\beta_k}{\pi_k}$ and
	subtract $\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2$ from both sides of~\eqref{eqn:simp-bundle-penal-merit-pf-2.5} to obtain
\begin{equation} \label{eqn:simp-bundle-penal-merit-pf-3}
  \centering
   \begin{aligned}
	   -\beta_k g_k^Td_k -\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2
	   \geq&  \beta_k \alpha_k\norm{d_k}^2 - \frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2 +\frac{\beta_k}{\pi_k}\sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k\\ 
	   \geq& \frac{1}{2}\alpha_k\beta_k\norm{d_k}^2 +\frac{\beta_k}{\pi_k}\sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k\\ 
	   =&  \frac{1}{2}\alpha_k\beta_k\norm{d_k}^2 +\frac{\beta_k}{\pi_k}  (\lambda^{k+1})^T \nabla c(x_k)^T d_k. 
   \end{aligned}
 \end{equation}
	On the other hand,~\eqref{eqn:simp-bundle-merit-penal-pf-1} together with~\eqref{eqn:simp-bundle-penal-merit-pf-3} imply that the merit function satisfies
\begin{equation*}% \label{eqn:simp-bundle-penal-merit-pf-4} 
 \centering
  \begin{aligned}
	  \phi_{1\pi_k}(x_k) - \phi_{1\pi_k}(x_{k+1})  =& r(x_k) -r(x_{k+1})+ \frac{1}{\pi_k}\norm{c(x_k)}_1
		    -\frac{1}{\pi_k}\norm{c(x_{k+1})}_1\\
			 >& -\beta_kg_k^T d_k-\frac{1}{2}\alpha_k\beta_k^2\norm{d_k}^2+ \frac{1}{\pi_k}\norm{c(x_k)}_1
		    -\frac{1}{\pi_k}\norm{c(x_{k+1})}_1\\
			\geq \frac{1}{2}\alpha_k\beta_k\norm{d_k}^2& +\frac{\beta_k}{\pi_k} (\lambda^{k+1})^T \nabla c(x_k)^T d_k		  +  \frac{1}{\pi_k}\norm{c(x_k)}_1 -\frac{1}{\pi_k}\norm{c(x_{k+1})}_1. \\
  \end{aligned}
\end{equation*}
The above inequality and the line search condition~\eqref{eqn:line-search-cond-penal} lead to
\begin{equation*} \label{eqn:simp-bundle-penal-merit-pf-5}
 \centering
  \begin{aligned}
	  \phi_{1\pi_k}(x_k) - \phi_{1\pi_k}(x_{k+1})  
			 >\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2-\eta_{\beta}\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2
			 =(1-\eta_{\beta})\frac{1}{2}\alpha_k\beta_k\norm{d_k}^2,
  \end{aligned}
\end{equation*}
which proves that $x_{k+1}$ is a descent step for $\phi_{1\pi_k}(\cdot)$. In addition, let $\bar{\pi}$ be the stabilized value for $\pi_k$,~\eqref{eqn:simp-bundle-fea-c-ls-pf-5} implies
\begin{equation*}% \label{eqn:simp-bundle-penal-merit-pf-6}
 \centering
  \begin{aligned}
	  \beta_k \geq \frac{1}{2} ^{\lceil \log_{\frac{1}{2}} \frac{\eta_{\beta} \alpha_0 \bar{\pi}}{2m H^c_u} \rceil}:=\bar{\beta}^{\pi}.
  \end{aligned}
\end{equation*}
Thus, %from~\eqref{eqn:simp-bundle-penal-merit-pf-5},
$\phi_{1\pi_k}(x_k)-\phi_{1\pi_k}(x_{k+1})> c_{\phi}^{\pi} \norm{d_k}^2$, where $c_{\phi}^{\pi} = (1-\eta_{\beta})\frac{1}{2}\alpha_0 \bar{\beta}^{\pi}>0$ for all $k$.
%Or equivalently, there exists $c_{\phi}^{\pi}>0$ such that $\phi_{1\pi_k}(x_k)-\phi_{1\pi_k}(x_{k+1})>c_{\phi}^{\pi}\norm{d_k}^2$.
\end{proof}
In general, the global convergence analysis from Section~\ref{sec:alg-convg} stands when $\pi_k$ is bounded away from $0$ and $\theta_k$ is bounded. This is reflected in the following two theorems, which are similar to Theorem~\ref{thm:simp-KKT}.
%, where we again uses LICQ to bound $\lambda^k$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:simp-KKT-consistency-finite}
	Under the Assumptions~\ref{assp:upperC2} and~\ref{assp:boundedHc} and LICQ conditions of Lemma~\ref{lem:bounded-lp}, if Algorithm~\ref{alg:simp-bundle-const} is called finitely many times, then every accumulation point of the serious point sequence $\{x_k\}$ generated from Algorithms~\ref{alg:simp-bundle}
	and~\ref{alg:simp-bundle-const} is a KKT point of problem~\eqref{eqn:opt-ms-simp}. 
\end{theorem}
%The proof is similar to that of Theorem~\ref{thm:simp-KKT}. % and straightforward.
Since there are only a finite number of consistency restoration steps, the linearized constraints become consistent for $k$ large enough. Thus, only Algorithm~\ref{alg:simp-bundle} is called for $k$ large enough. As a result, Theorem~\ref{thm:simp-KKT-consistency-finite} is a direct consequence of Theorem~\ref{thm:simp-KKT}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:simp-KKT-consistency-bounded}
	Under Assumptions~\ref{assp:upperC2},~\ref{assp:boundedHc} and LICQ conditions of Lemma~\ref{lem:bounded-lp}, if Algorithm~\ref{alg:simp-bundle-const} is called infinitely many times with nonzero stabilized penalty parameter, \textit{i.e.}, $\pi_t=\pi_k > 0$ for all $t\geq k$,
	then any accumulation point of the serious point sequence $\{x_k\}$ generated by Algorithms~\ref{alg:simp-bundle} 
	and~\ref{alg:simp-bundle-const}
	is either a KKT point of~\eqref{eqn:opt-ms-simp} or a critical point 
	of the linearized constraint violation of $c$. 
\end{theorem}
The proof is similar to that of Theorem~\ref{thm:simp-KKT} and we only provide a succinct discussion here.
First, by Lemma~\ref{lem:sufficientdecrease-penal} we have that $\alpha_t = \alpha_k$ for all $t\geq k$ and all steps produced by both algorithms are serious steps.
We note that by design both penalty parameters $\theta_k$ and $\frac{1}{\pi_k}$ in~\eqref{eqn:opt-ms-simp-bundle-merit} and~\eqref{def:merit-fea} are monotonically nondecreasing across iterations and algorithms. By Lemma~\ref{lem:bounded-lp}, $\lambda^k$ is bounded. Given a nonzero stabilized $\pi_k$, $\theta_k$ is bounded and remains constant from step 7 in Algorithm~\ref{alg:simp-bundle}.
Together with step 6 in Algorithm~\ref{alg:simp-bundle-const}, the merit functions $\phi_{1\theta_k}(\cdot)$ of~\eqref{eqn:opt-ms-simp-bundle-merit} and  $\phi_{1\pi_k}(\cdot)$  of~\eqref{def:merit-fea} have the same parameter $\theta_k=\frac{1}{\pi_k}:=\bar{\theta}$
, where $\bar{\theta}$ is the stabilized value.
By Lemma~\ref{lem:sufficientdecrease-merit} and~\ref{lem:sufficientdecrease-merit-penal}, $\{\phi_{1\pi_k}(x_k)\}$ and $\{\phi_{1\theta_k}(x_k)\}$ decrease monotonically in the order of $\norm{d_k}^2$ and are bounded below. Therefore, they converge and $\{d_k\}$ generated by both algorithms satisfies $d_k \to 0$.

Compared to Theorem~\ref{thm:simp-KKT-consistency-finite}, Theorem~\ref{thm:simp-KKT-consistency-bounded} leaves the possibility that after a finite number of calls of Algorithm~\ref{alg:simp-bundle}, only the consistency restoration Algorithm~\ref{alg:simp-bundle-const} is invoked; in this case an accumulation point of $\{x_k\}$ is not guaranteed to be a KKT point. This can be seen from the constraints of the penalty problem~\eqref{eqn:opt-ms-simp-bundle-penal} where $v$ or $w$ could be nonzero even as $d_k\to 0$. 
However, if an accumulation point $\bar{x}$ is feasible, \textit{i.e.}, $c(\bar{x}) = 0$, then it is indeed a KKT point of problem~\eqref{eqn:opt-ms-simp}, the proof of which is the same as in Theorem~\ref{thm:simp-KKT} at this point. 
Otherwise, if $\bar{x}$ is infeasible, %\textit{i.e.}, $c(\bar{x})\neq 0$, it is not a KKT point. 
%Meanwhile,
from~\eqref{def:pd-penal} and $d_k\to 0$, we have $\delta_k^{\pi_k}\to 0$. 
From step 6 in Algorithm~\ref{alg:simp-bundle-const}, the update rule of $\pi_k$ enforces $\eta_f \delta_k^f\leq \delta_k^{\pi_k}$. Therefore, with a constant parameter $\eta_f$, we obtain $\delta_k^f\to 0$.
Hence, an infeasible $\bar{x}$ is a critical point of linearized constraint violation of $c$. 
This convergence result is similar to the exact penalty method for smooth objectives~\cite{Nocedal_book}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Finally, the following theorem covers the case when the penalty parameter $\pi_k \to 0$.
\begin{theorem}\label{thm:simp-KKT-consistency-unbounded}
	Under Assumptions~\ref{assp:upperC2},~\ref{assp:boundedHc} and LICQ conditions of Lemma~\ref{lem:bounded-lp}, if Algorithm~\ref{alg:simp-bundle-const} is called
	infinite many times and $\pi_k \to 0$,
	then an accumulation point of the serious point sequence $\{x_k\}$ generated from Algorithm~\ref{alg:simp-bundle}
	and~\ref{alg:simp-bundle-const}
	is a critical point of the linearized constraint violation of $c$. 
\end{theorem}
\begin{proof}
	Lemma~\ref{lem:bounded-lp} implies that the Lagrange multipliers from Algorithm~\ref{alg:simp-bundle} are bounded. Therefore, a $\pi_k\to 0$ is caused by step 6 in Algorithm~\ref{alg:simp-bundle-const} being called infinitely many times which in turn increases $\theta_k$ as well. 
	Because we are considering an infinite number of iterations where $\delta_k^f>0$ (otherwise the algorithm would have terminated at step 3), the number of loops 
	between step 5 and 6 is finite for each $k$ by Lemma~\ref{lem:consistency-penal-defined}. Thus, to have infinitely many steps 6, we must have an infinite number 
	of iterations that would enter step 6 at least once.
	Let $k$ be one of the iterations where $\pi_k$ is reduced through step 6
	and denote $\pi_k^0 = \min{(\pi_{k-1},\frac{1}{\theta_k})}$ as the penalty parameter after step 1.
	Then, the change in objective of problem~\eqref{eqn:opt-ms-simp-bundle-penal} with $\pi_{k}^0$ is 
	\begin{equation}
          \centering
	  \begin{aligned}
		  \delta_k^{0} = \pi_{k}^0 \left(-g_k^T d_k^{0} -\frac{1}{2}\alpha_k \norm{d_k^{0}}^2\right) +\norm{c(x_k)}_1-\norm{c(x_k) +\nabla c(x_k)^T d_k^{0}}_1, 
          \end{aligned}
	\end{equation}
	where $d_k^{0}$ is the solution of~\eqref{eqn:opt-ms-simp-bundle-penal} with $\pi_{k}^0$.
		Since $\pi_{k}^0 $ enters step 6 in Algorithm~\ref{alg:simp-bundle-const}, we have that $\delta_k^{0} < \eta_f\delta_k^f$. 
	Using the definition~\eqref{def:pd-fea} of $\delta_k^f$, we write
   \begin{equation*} %\label{eqn:simp-bundle-fea-pi-0-1}
   \centering
    \begin{aligned}
	    \eta_f\delta_k^f > \delta_k^{0} %=& \pi_{k}^0\left(-g_k^T d_k^{0} -\frac{1}{2}\alpha_k \norm{d_k^{0}}^2\right) +\norm{c(x_k)}_1- \norm{c_j(x_k)+ \nabla c_j(x_k)^T d_k^{0}}_1\\
	      \geq& \pi_{k}^0\left(-g_k^T d_k^f -\frac{1}{2}\alpha_k \norm{d_k^f}^2\right) +\norm{c(x_k)}_1- \norm{c(x_k)+ \nabla c(x_k)^T d_k^f}_1\\
		     =& \pi_{k}^0\left(-g_k^T d_k^f  - \frac{1}{2} \alpha_k \norm{d_k^f}^2\right) + \delta_k^f \\
		     \geq& \pi_{k}^0\left(-\norm{g_k}\norm{d_k^f} - \frac{1}{2}\alpha_k\norm{d_k^f}^2\right)+ \delta_k^f.\\
    \end{aligned}
   \end{equation*}
	Since $x_k$, $g_k$, and $\alpha_k$ are bounded, by denoting $D = \norm{d_u^k-d_l^k}=\norm{x_u}$, we have 
   \begin{equation*}% \label{eqn:simp-bundle-fea-pi-0-2}
   \centering
    \begin{aligned}
	    (1-\eta_f) \delta_k^f \leq& \pi_{k}^0 \left(\norm{g_k}\norm{d_k^f} + \frac{1}{2}\alpha_k\norm{d_k^f}^2\right)
			       \leq  \pi_{k}^0\left( \norm{g_k} D + \frac{1}{2}\alpha_k D^2 \right).\\
    \end{aligned}
   \end{equation*}
	Therefore, as $\pi_k \to 0$ and, thus, $\pi_k^0\to 0$, so does $\delta_k^f$.
	Given an accumulation point $\bar{x}$, let $x_{k_s}\to\bar{x}$ be a subsequence of $\{x_k\}$, we have $\delta_{k_s}^f \to 0$. This completes the proof.
\end{proof}

Theorem~\ref{thm:simp-KKT-consistency-unbounded} %is a relatively weak result in the sense that it 
does not distinguish between feasible and infeasible accumulation points $\bar{x}$. 
For smooth optimization, stronger results are possible even under a  
less restrictive constraint qualification, Mangasarian–Fromovitz constraint qualification; for example, Byrd et al.~\cite{byrd2005} show that if $\pi_k \to 0$ and $c(\bar{x}) = 0$, then their SLQP algorithm converges 
to a KKT point. Such result for (nonsmooth) upper-$C^2$ objective function is not evident to us and will be the subject of our future research. 



